On Reinforcement Learning and Distribution Matching for Fine-Tuning Language Models with no Catastrophic Forgetting

The availability of large pre-trained models is changing the landscape of Machine Learning research and practice, moving from a training-from-scratch to a fine-tuning paradigm. While in some applications the goal is to "nudge" the pre-trained distribution towards preferred outputs, in others it is to steer it towards a different distribution over the sample space. Two main paradigms have emerged to tackle this challenge: Reward Maximization (RM) and, more recently, Distribution Matching (DM). RM applies standard Reinforcement Learning (RL) techniques, such as Policy Gradients, to gradually increase the reward signal. DM prescribes to first make explicit the target distribution that the model is fine-tuned to approximate. Here we explore the theoretical connections between the two paradigms, and show that methods such as KL-control developed for RM can also be construed as belonging to DM. We further observe that while DM differs from RM, it can suffer from similar training difficulties, such as high gradient variance. We leverage connections between the two paradigms to import the concept of baseline into DM methods. We empirically validate the benefits of adding a baseline on an array of controllable language generation tasks such as constraining topic, sentiment, and gender distributions in texts sampled from a language model. We observe superior performance in terms of constraint satisfaction, stability and sample efficiency.

==> RMvsDM NeurIPS 2022 Submission-5/checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{section:discussion}}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix \ref{section:Broader}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{In Appendix \ref{appendix:baselines} we present proofs of all mathematical facts referred to in the paper.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is included as supplementary material available to the reviewers and area chairs and will be made publicly available alongside the camera ready version of the paper.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Appendix \ref{appendix:Hyperparameters} we provide the hyperparameters used throughout our experiments and report our hardware configuration. In Appendix \ref{detailed-metrics}, we describe in detail how $\KL(p, \pit)$ and $\TVD(p, \pit)$ were estimated and provide an extended pseudocode for our training loop in Algorithm~\ref{appendix:al:DPG}. }
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{However, we found the variance across random seeds to be negligible and not comparing across random seeds is a standard practice when working with large language models where the cost of a single run is significant.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In Appendix \ref{appendix:Hyperparameters} we report our hardware configuration.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In Appendix \ref{appendix:Hyperparameters}.}
  \item Did you mention the license of the assets?
    \answerYes{In Appendix \ref{appendix:Hyperparameters}.}
  \item Did you include any new assets either in the supplemental material or as a URL? \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> RMvsDM NeurIPS 2022 Submission-5/figures/algorithm1.tex <==
\begin{wrapfigure}{r}{0.53\textwidth}
\begin{minipage}{0.53\textwidth}
\vspace{-13px}
\begin{algorithm}[H]
\caption{KL-Adaptive DPG  \textcolor{blue}{with baseline} \label{al:KL-adaptive-DPG-baseline}}
\begin{small}
\begin{algorithmic}[1]
\Require $P$, initial generative model $a$
\State $\pi_\theta \gets a$, $q \gets a$
\For{each iteration}
\For{each episode}
    \State sample $x$ from $q(\cdot)$
    \State $\theta \gets \theta + \alpha^{(\theta)} \textcolor{blue}{\Big[ \textcolor{black}{\frac{P(x)}{q(x)}} - Z\frac{\pit(x)}{q(x)} \Big]} \ \nabla_\theta \log \pi_\theta(x)$ 
\EndFor
\If{ $\KL(p||\pi_\theta) <  \KL(p||q)$} 
    \State $q \gets \pi_\theta$
\EndIf
\EndFor
\Ensure $\pi_\theta$
\end{algorithmic}
\end{small}
\end{algorithm}
\vspace{-20px}
\end{minipage}
\end{wrapfigure}

==> RMvsDM NeurIPS 2022 Submission-5/figures/tab_RLvsDPG.tex <==

\begin{table*}[t]
    \centering
    \small
    \vspace{-0.5cm}
\begin{tabular}{lll}
\toprule
 & \textbf{Policy Gradients} & \textbf{\DPG}\\
\midrule
 \textbf{Reward} & 
 $R(x)$   & 
 $R_\theta(x) =\frac{P(x)}{\pi_\theta(x)}$ \\
 \addlinespace
%   \textbf{Advantage} & 
%  $R(x) - [\E_{x \sim\pit} R(x)]$ & 
%  $\frac{P(x)}{\pi_\theta(x)} - Z$ \\
 \textbf{ $\nabla_\theta$} & 
{\small $\E_{x \sim \pit} R(x) \nabt \log \pit(x)$} & 
{\small $\E_{x \sim \pit} \frac{P(x)}{\pi_\theta(x)} \nabt \log \pit(x)$} \\
 \addlinespace
 \textbf{Baseline}& 
 $\E_{x \sim\pit} R(x)$  & 
 $Z$   \\
\addlinespace
 \textbf{ $\nabla_\theta$ with Baseline } & 
 {\small $\E_{x \sim \pit} \Big[R(x) - \E_{x \sim\pit} R(x) \Big] \nabt \log \pit(x)$} & 
{\small $\E_{x \sim \pit} \Big[ \frac{P(x)}{\pi_\theta(x)} - Z \Big] \nabt \log \pit(x)$} \\
\bottomrule
\end{tabular}
    \caption{\small{A comparison between Policy Gradients~\citep{sutton_policy_gradients} and Distributional Policy Gradients~\citep{opt-rl-arxiv-2019} forms of Reward, Baseline, and Gradient of the loss function (the PG-term) before ($\nabla_\theta$) and after ($\nabla_\theta$ with Baseline) including a baseline for variance reduction .}}
    \label{tab:comparison_DPGvsPG}
\end{table*}

==> RMvsDM NeurIPS 2022 Submission-5/figures/table_bsz_experiments.tex <==
\begin{table}
\tiny
\begin{tabular}{lllrrrrrrrrr}
\toprule
             &      &      &  b(x) &  KL(p, pi) &  KL(pi, a) &  Dist-1 &  Dist-2 &  Dist-3 &  SB-3 &  SB-4 &  SB-5 \\
             & batch size & method &      &        &        &       &       &       &        &        &        \\
\midrule
word amazing & 0    & a & 0.00 &   6.46 &  -0.00 &  0.87 &  0.95 &  0.93 &   0.96 &   0.90 &   0.82 \\
             & 256  & GDC++ & 0.72 &   3.94 &   7.28 &  0.87 &  0.95 &  0.94 &   0.97 &   0.94 &   0.88 \\
             &      & GDC & 0.59 &   4.61 &   8.34 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             \
             & 512  & GDC++ & 0.72 &   2.57 &   5.34 &  0.86 &  0.95 &  0.93 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.69 &   2.40 &   5.36 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 1024 & GDC++ & 0.75 &   1.34 &   4.71 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.73 &   1.89 &   4.70 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 2048 & GDC++ & 0.73 &   1.35 &   4.33 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.71 &   1.46 &   4.40 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
\bottomrule
Multiple Dist & 0    & a & 0.12 &   0.16 &   0.00 &  0.90 &  0.95 &  0.92 &   0.98 &   0.94 &   0.90 \\
             & 256  & GDC++ & 0.24 &   0.65 &   1.06 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.52 &   1.04 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 512  & GDC++ & 0.24 &   0.37 &   0.78 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.36 &   0.88 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 1024 & GDC++ & 0.24 &   0.20 &   0.75 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.24 &   0.81 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 2048 & GDC++ & 0.24 &   0.20 &   0.68 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.22 &   0.70 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\

\bottomrule
\end{tabular}
\end{table}


==> RMvsDM NeurIPS 2022 Submission-5/figures/table_pointwise_dist_experiments.tex <==
\begin{table}[H]
\tiny
\centering
\begin{tabular}{llcccccccc}
\toprule
 &   &  &  \multicolumn{2}{c}{\textbf{Fluency}} & \multicolumn{3}{c}{\textbf{Sentence Level Diversity}} &  \multicolumn{2}{l}{\textbf{Corpus Level Diversity}} \\
& \textbf{Method}  &  \textbf{Ctrl ($\uparrow$)} & \textbf{KL{(p,$\boldsymbol{\pi}$)}} ($\downarrow$) &  \textbf{KL(pi,a)} ($\downarrow$)&  \textbf{Dist-1} ($\uparrow$)&  \textbf{Dist-2} ($\uparrow$)&  \textbf{Dist-3} ($\uparrow$)&  \textbf{SB-4} ($\downarrow$)&  \textbf{SB-5}($\downarrow$) \\
\midrule
\multicolumn{10}{c}{\textbf{Pointwise Constraints Experiments}}\\
\midrule
Word Amazing 
 & \gc{Original LM} &  \gc{0.00} &  \gc{6.02} &  \gc{0.00} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.82} \\
 & Reinforce &  \r{1.00} &  \r{134.31} & \r{78.39} &  \r{0.69} &  \r{0.91} &  \r{0.94} &  \r{0.98} &  \r{0.96} \\
 & Ziegler &  \textbf{0.82} &  4.56 &  5.88 &  0.86 &  0.95 &  0.94 &  0.94&  0.88 \\
 & GDC &  0.65 &  2.57 &  5.06 &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
 & GDC++ (Ours)&  \underline{0.69} &  \underline{\textbf{2.10}} &  \underline{\textbf{4.74}} &  \underline{\textbf{0.87}} &  0.95 &  0.94 &  0.93 &  0.87 \\
   \midrule
Word WikiLeaks 
 & \gc{Original LM} &  \gc{0.00} &  \gc{8.54} &  \gc{0.00} &  \gc{0.86} &  \gc{0.9}4 &  \gc{0.92} &  \gc{0.89} &  \gc{0.80} \\
 & Reinforce &  \r{1.00}&  \r{8.00} &  \r{117.24} &  \r{0.38} &  \r{0.56} & \r{0.64} & \r{0.98} &  \r{0.97} \\
 & Ziegler &  0.68 &  0.00 &  6.03 &  0.87 &  0.96 &  0.94 &  0.95 &  0.90 \\
 & GDC &  0.75 &  3.22 &  7.96 &  0.88 &  0.96 &  0.94 &   0.95 &  0.90 \\
 & GDC++ (Ours) &    \underline{\textbf{0.77}} &  \underline{\textbf{2.21}} &  \underline{\textbf{7.53}} &  0.88 &  0.96 &  0.94 &  0.95 &  0.91 \\
  \midrule
Wordlist Science 
 & \gc{Original LM} &  \gc{0.06} & \gc{2.79} & \gc{0.00} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce&  \r{1.00} &  \r{140.02} &  \r{66.68} &  \r{0.29} &  \r{0.41} &  \r{0.49} & \r{0.98} &   \r{0.97} \\
  & Ziegler &  \textbf{1.00} &    6.1 &  5.88 &  0.86 &  0.95 &  0.93 &  0.95 &  0.90\\
 & GDC &  0.52 &  2.27 &  2.89 &  0.86 &  0.95 &  0.93 &  0.93 &  0.87 \\
 & GDC++ (Ours) &  \underline{0.54} &  \underline{1.78} &  \underline{\textbf{2.11}} &  0.86 &  0.95 &  0.93 & \underline{\textbf{0.92}} &  \underline{\textbf{0.86}} \\
  \midrule
Wordlist Politics 
 & \gc{Original LM} &  \gc{0.07} &  \gc{2.65} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce&  \r{1.00} &  \r{263.79} &  \r{65.06} &  \r{0.26} &  \r{0.40} &  \r{0.51}& \r{0.98} &  \r{0.97} \\
 & Ziegler &  \textbf{1.00} &  8.46 &  5.92 &  0.87 &  0.96 &  0.94 &  0.96 &  0.92 \\
 & GDC &  \underline{0.58} &  2.70 &  2.49 &  0.87 &  \underline{0.96} &  \underline{0.94} &  0.93 &  0.88 \\
 & GDC++ (Ours) &  0.49 &  \underline{\textbf{2.01}} &  \underline{\textbf{1.35}} &  0.87 &  0.95 &  0.93 &  0.93 &  \underline{\textbf{0.87}} \\
  \midrule
+ve Sentiment 
 & \gc{Original LM} &  \gc{0.17} &  \gc{2.06} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.93} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce &  \r{1.00} &  \r{153.75} &  \r{80.07} &  \r{0.27} &  \r{0.37} &  \r{0.41} &  \r{0.97} &  \r{0.95} \\
 & Ziegler &  \textbf{0.98} &  5.70 &  5.98 &  0.85 &  0.96 &  0.94 &   0.96 &  0.91 \\
 & GDC &  0.59 &  1.68 &  1.89 &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
 & GDC++ (Ours) &  \underline{0.60} &  \underline{\textbf{1.67}} &  \underline{\textbf{1.88}} &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
  \midrule
-ve Sentiment 
 & \gc{Original LM} &  \gc{0.13} &  \gc{2.14} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &   \gc{0.90} &  \gc{0.82} \\
 & Reinforce &  \r{1.00} &  \r{88.48} &  \r{70.38} &  \r{0.83} &  \r{0.96} &  \r{0.94} &  \r{0.97} &  \r{0.93} \\
 & Ziegler &  0.95 &  6.12 &  6.00 &  0.84 &  0.95 &  0.94 &  0.96 &  0.92 \\
 & GDC &  \underline{0.52} &  1.72 &  1.79 &  0.86 &  0.95 &  0.94 &  0.94 &  0.88 \\
 & GDC++ (Ours) &  0.51 &  \underline{\textbf{1.66}} &  \underline{\textbf{1.63}} &  0.86 &  0.95 &  0.94 & \underline{\textbf{0.93}} &  0.88 \\
  \midrule
  \multicolumn{10}{c}{\textbf{Distributional Constraints Experiments}}\\
  \midrule
Single 
 & \gc{Original LM} &  \gc{0.19} &  \gc{0.39} &  \gc{0.01} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  0.80 &  0.74 &  0.71 &  0.89 &  0.95 &  0.92 &  0.95 &  0.90 \\
 & GDC++ (Ours) &  \underline{\textbf{0.81}} &  \underline{\textbf{0.33}} &  \underline{\textbf{0.66}} &  0.89 &  0.95 &  0.92 &  \underline{\textbf{0.94}} &  0.90 \\
  \midrule
Multiple 
 & \gc{Original LM} &  \gc{0.49} &  \gc{0.40} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  0.92 &  0.53 &  0.85 &  0.90 &  0.95 &  0.92 &  0.95 &  0.90 \\
 & GDC++ (Ours) &  \underline{\textbf{0.95}} &  \underline{\textbf{0.30}} &  \underline{\textbf{0.76}} &  0.90 &  0.95 &  0.92 &  0.95 &  0.90 \\
  \midrule
Hybrid Sports 
 & \gc{Original LM} &  \gc{0.22} &  \gc{0.20} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  \underline{\textbf{0.87}} &  \underline{\textbf{0.24}} &  2.65 &  0.93 &  0.95 &  0.92 &  0.96 &  0.92 \\
 & GDC++ (Ours) &  0.85 &  0.87 &  \underline{\textbf{2.35}} &  0.93 &  0.95 &  0.92 &  0.96 &  0.92 \\
  \midrule
Hybrid Science 
 & \gc{Original LM} &  \gc{0.09} &  \gc{0.00} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.89} \\
 & GDC &  0.68 &  1.52 &  3.92 &  0.88 &  0.95 &  0.91 &  0.95 &  0.92 \\
 & GDC++ (Ours) &  \underline{\textbf{0.70}} &  \underline{\textbf{1.41}} &  \underline{\textbf{3.83}} &  0.88 &  0.95 &  \underline{\textbf{0.92}} &  0.95 &  \underline{\textbf{0.91}} \\
%   \midrule
% avg & GDC &  0.55 &  1.74 &  2.92 &  0.88 &  0.95 &  0.93 &  0.97 &  0.94 &  0.89 \\
%  & GDC++ (Ours) &  0.54 &  1.43 &  2.68 &  0.88 &  0.95 &  0.93 &  0.97 &  0.94 &  0.89 \\
%  & Original LM &  0.09 &  2.52 &  0.00 &  0.88 &  0.95 &  0.92 &  0.96 &  0.91 &  0.85 \\
%  & Reinforce &  1.00 &  131.39 &  79.64 &  0.45 &  0.60 &  0.65 &  0.99 &  0.98 &  0.96 \\
%  & Ziegler &  0.89 &  4.97 &  5.96 &  0.86 &  0.96 &  0.94 &  0.98 &  0.95 &  0.91 \\
\bottomrule
\vspace{5px}
\end{tabular}
\caption{
\small{
%   Evaluation metrics:  $\KL(p, \pi_{\theta})$ ($\downarrow$ better), $\mathbb{E}_{\pit} \phi(x)$ ($\uparrow$ better), $\KL(\pi_{\theta}, a)$ ($\downarrow$ better), Self-BLEU-5 ($\downarrow$ better), and Distinct-1 ($\uparrow$ better) aggregated over 6 pointwise constraints experiments (tasks 1-6) for policies obtained from GDC\texttt{++}, GDC, Ziegler and Reinforce. See Figure~\ref{fig:distributional-compare-methods-metrics} for aggregated distributional constraints experiments, and Figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} in the Appendix for a detailed view on each experiment.
      Evaluation over 6 pointwise constraints experiments (tasks 1-6) and 4 distributional constraints experiments (tasks 7-10) for policies obtained from GDC\texttt{++} (ours), GDC, Ziegler and Reinforce.
      See figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} in the Appendix for a detailed view on each experiment.
    %   $\KL(p, \pi_{\theta})$ ($\downarrow$ better), $\mathbb{E}_{\pit} \phi(x)$ ($\uparrow$ better), $\KL(\pi_{\theta}, a)$ ($\downarrow$ better), Self-BLEU-5 ($\downarrow$ better), and Distinct-n ($\uparrow$ better).
      Results of the initial policy (\gc{Original LM}) are displayed for reference.The best method (excluding ties) overall is highlighted in \textbf{bold}, while the best method between GDC and GDC++ is \underline{underlined}. Runs that suffer degeneration due to \r{catastrophic forgetting} (measured by sequence level repetitions) are highlighted in red and excluded from best method comparison. Our method GDC++ that includes a baseline for variance reduction, outperforms GDC \citep{khalifa_2021} in 7/10 tasks in terms of control satisfaction rate (\textbf{Ctrl}), as well as convergence towards the optimal policy (\textbf{KL{(p,$\boldsymbol{\pi}$)}}) and distance from the original LM (\textbf{KL(pi,a)}) in 10/10 of the tasks. 
   }
   }
   \label{tab:all_experiments_results}
\end{table}



==> RMvsDM NeurIPS 2022 Submission-5/math_commands.tex <==
\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\KLhat}{\hat{D}_{\mathrm{KL}}}
\newcommand{\TVD}{\mathrm{TVD}}
\newcommand{\CE}{\mathrm{CE}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\pit}{{\pi_\theta}}
\newcommand{\nablapitlog}{\nabla_{\theta} \log \pit(x)}
\newcommand{\sprod}[2]{{\left<#1,#2\right>}}
\newcommand{\Rtz}{\Rt} %R_\theta Ziegler
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\BibTeX{B\textsc{ib}\TeX}
\newcommand{\GDC}{GDC }
\newcommand{\GDCon}{GDC\textsuperscript{on} }
\newcommand{\GDCoff}{GDC\textsuperscript{off} }
\newcommand{\GDCplus}{GDC\texttt{++} }
\newcommand{\DPG}{DPG }
\newcommand{\DPGon}{DPG\textsuperscript{on} }
\newcommand{\DPGoff}{DPG\textsuperscript{off} }

\newcommand{\Ron}{R^\text{ on}_\theta(x)}
\newcommand{\Roff}{R^\text{ off}_\theta(x)}
\newcommand{\Aon}{A^\text{ on}_\theta(x)}
\newcommand{\Aoff}{A^\text{ off}_\theta(x)}
\newcommand{\ARL}{A^\text{ RL}_\theta(x)}
\newcommand{\Bon}{B^\text{on}(x)}
\newcommand{\Boff}{B^\text{off}(x)}
\newcommand{\BRL}{B^\text{RL}(x)}


\newcommand{\grad}{G_\theta}
\newcommand{\gradest}{G(\theta)}
\newcommand{\vargrad}{\mathrm{Var}(\grad)}
\newcommand{\mgrad}{\mathbf{\mu}(\grad)}

\newcommand{\Adv}{\mathrm{A}}
\newcommand{\mAdv}{\mu^\Adv}
\newcommand{\mAbsAdv}{\mu^{|\Adv|}}
\newcommand{\varAdv}{\mathrm{Var}\left(\Adv\right)}

\newcommand{\nabt}{\nabla_\theta}
\newcommand{\Rt}{R_\theta}

\newcommand{\EX}[1]{\E_{#1}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\newif\ifready
% \readytrue: ready-to-submit version
%\readyfalse: commented version

% \readyfalse
\readytrue

\ifready
\newcommand{\ftk}[1]{}
\newcommand{\fgk}[1]{}
\newcommand{\fmd}[1]{}
\newcommand{\ptmd}[1]{#1}
\newcommand{\ptgk}[1]{#1}
\newcommand{\fhe}[1]{}
\newcommand{\annot}[1]{}
\else
\newcommand{\ftk}[1]{{\color{red}\footnote{\textcolor{red}{TK: #1}}}}
\newcommand{\fgk}[1]{{\color{orange}\footnote{\textcolor{orange}{GK: #1}}}}
\newcommand{\fmd}[1]{{\color{blue}\footnote{\textcolor{blue}{MD: #1}}}}
%%% \ptmd : proposed text md
\newcommand{\ptmd}[1]{\textcolor{blue}{#1}}
\newcommand{\ptmd}[1]{\textcolor{orange}{#1}}
%%%
\newcommand{\fhe}[1]{{\color{olive}\footnote{\textcolor{olive}{HE: #1}}}}
\newcommand{\annot}[1]{\textbf{\textcolor{purple}{#1~}}}
\fi

% MD 11/10/2022
\newif\ifreadyII
% \readyIItrue: Version submitted After Rebuttal
%\readyIIfalse: commented version

% \readyIIfalse
\readyIItrue

\ifreadyII
\newcommand{\ftkII}[1]{}
\newcommand{\fgkII}[1]{}
\newcommand{\fmdII}[1]{}
\newcommand{\ptmdII}[1]{#1}
\newcommand{\ptgkII}[1]{#1}
\newcommand{\fheII}[1]{}
\newcommand{\annotII}[1]{}
\else
\newcommand{\ftkII}[1]{{\color{red}\footnote{\textcolor{red}{TK: #1}}}}
\newcommand{\fgkII}[1]{{\color{orange}\footnote{\textcolor{orange}{GK: #1}}}}
\newcommand{\fmdII}[1]{{\color{blue}\footnote{\textcolor{blue}{MD: #1}}}}
%%% \ptmd : proposed text md
\newcommand{\ptmdII}[1]{\textcolor{blue}{#1}}
\newcommand{\ptheII}[1]{\textcolor{orange}{#1}}
%%%
\newcommand{\fheII}[1]{{\color{olive}\footnote{\textcolor{olive}{HE: #1}}}}
\newcommand{\annotII}[1]{\textbf{\textcolor{purple}{#1~}}}
\fi










% MD 31/07/2022
\newif\ifreadyAR
% \readyARtrue: Version submitted After Rebuttal
%\readyARfalse: commented version

% \readyARfalse
\readyARtrue

\ifreadyAR
\newcommand{\ftkAR}[1]{}
\newcommand{\fgkAR}[1]{}
\newcommand{\fmdAR}[1]{}
\newcommand{\ptmdAR}[1]{#1}
\newcommand{\ptgkAR}[1]{#1}
\newcommand{\fheAR}[1]{}
\newcommand{\annotAR}[1]{}
\else
\newcommand{\ftkAR}[1]{{\color{red}\footnote{\textcolor{red}{TK: #1}}}}
\newcommand{\fgkAR}[1]{{\color{orange}\footnote{\textcolor{orange}{GK: #1}}}}
\newcommand{\fmdAR}[1]{{\color{blue}\footnote{\textcolor{blue}{MD: #1}}}}
%%% \ptmd : proposed text md
\newcommand{\ptmdAR}[1]{\textcolor{blue}{#1}}
\newcommand{\ptheAR}[1]{\textcolor{orange}{#1}}
%%%
\newcommand{\fheAR}[1]{{\color{olive}\footnote{\textcolor{olive}{HE: #1}}}}
\newcommand{\annotAR}[1]{\textbf{\textcolor{purple}{#1~}}}
\fi




\newcommand{\Rtheta}{R_\theta}
\renewcommand{\Rtz}{R^z_\theta}
\newcommand{\Rpiz}{R^z_\pi}


\readyfalse
% \readytrue

% \ifready
% \newcommand{\fbe}[1]{}
% \newcommand{\fgk}[1]{}
% \newcommand{\fmd}[1]{}
% \newcommand{\fhe}[1]{}
% \newcommand{\annot}[1]{}
% \else
% \newcommand{\fbe}[1]{{\color{red}\footnote{\textcolor{red}{BE: #1}}}}
% \newcommand{\fgk}[1]{{\color{orange}\footnote{\textcolor{orange}{GK: #1}}}}
% \newcommand{\fmd}[1]{{\color{blue}\footnote{\textcolor{blue}{MD: #1}}}}
% \newcommand{\fhe}[1]{{\color{olive}\footnote{\textcolor{olive}{HE: #1}}}}
% \newcommand{\annot}[1]{\textbf{\textcolor{purple}{#1~}}}
% \fi

\newcommand{\smallparagraph}[1]{\textbf{#1}\hspace{1ex}}

==> RMvsDM NeurIPS 2022 Submission-5/sections/background.tex <==
%\setlength{\abovedisplayskip}{3pt}
%\setlength{\belowdisplayskip}{3pt}

\smallparagraph{Standard Policy Gradients}
\label{sec:pg}
One popular method for adapting the behaviour of language models to certain
% some
preferences has been that of assigning a ``reward'' score $R(x)$ for sequences $x$ sampled from an autoregressive language model (policy) $\pi_\theta$. 
Then, the simplest policy gradient algorithm in reinforcement learning, namely, REINFORCE \citep{Williams92}, 
% consists in finding 
aims to find
the policy $\pit(x)$ that maximizes the average reward $\EX{x \sim \pit} R(x)$, and this leads, via the so-called ``log derivative trick'', to a gradient ascent algorithm that iteratively samples $x$ from $\pit$ and update parameters by increments proportional to $R(x)\nabt \log \pit(x)$ via the following identity:
\begin{align}
  \label{eq:REINFORCE}
  \nabt \EX{x \sim \pit} R(x) &= \EX{x \sim \pit} R(x) \nabt \log \pit(x).
\end{align}


\smallparagraph{KL-control}
\label{sec:kl_control}
% In the context of finetuning large language models, reward maximization objectives have often been criticized for their large deviations from the original pre-trained language models. 
% This ``catastrophic forgetting'' effect leads to poor generated sequences that improve the average reward at the expense of coherence, fluency and sample diversity~\citep{LiuLSNCP16,Wu_googleMT16,khalifa_2021}.
~\citep{todorov,kappen2012optimal}, was leveraged by \cite{Jaques-2017,KL_jaquesK19} and \cite{Ziegler19} to include a KL penalty term in the reward function to penalize large deviations from the original pretrained model $a(x)$, weighted by a free hyperparameter $\beta$ to control the trade-off between the two goals.
% i.e. maximizing 
That is, they maximize
the expectation $\E_{x \sim \pit} \Rtz(x)$, where:
\begin{align}
  \Rtz(x)\doteq r(x) - \beta \log \frac{\pit(x)}{a(x)}.
  \label{RTZ_first_mention}
\end{align} 

%If we define $\Rtheta(x) \doteq \frac{P(x)}{\pit(x)}$,%
%\fmd{I am simplifying the notation from $\Ron$ to $\Rtheta$ here to avoid cluttering already delicate explanations. $\Ron$ can be defined later.}
%the right-hand sides of \eqref{eq:dpgon} and \eqref{eq:REINFORCE} look almost identical. So, are there any differences between DPG and standard Policy Gradients?

\smallparagraph{Distributional Policy Gradients}
\label{sec:dpg}
%An EBM such as $P$ in \eqref{eq:target-EBM}, as well as its normalized form $p$, can compute scores associated to a sequence $x$, but are not directly usable for sampling.
%This is due to two factors: (i) the partition function $Z$ is not directly known and can be difficult to estimate, making $p(x)$ not obvious to compute\fgk{This sounds in contradiction with the fact that we rely on easily computing it through IS \textcolor{red}{TK: Yes, I'd just say $P(x)$ can't be sampled from directly}}, (ii) there is a huge gap between computing $p(x)$ for each \emph{individual} $x$ and being able to \emph{sample} from $p$. 
%
% A different solution to the problem of controlled text generation was given by \citet{khalifa_2021}.
% There, the authors disentangle the problems of defining \emph{what} is the optimal desired distribution from \emph{how} a model that approximates this distribution is actually learned. Specifically, the authors define an optimal distribution as an unnormalized probability distribution or EBM $P(x)$.
%
(DPG)~\citep{opt-rl-arxiv-2019} is 
% the 
\ptmd{a recent}
approach used to fit an autoregressive policy $\pit$ to the distribution $p(x)=P(x)/Z$ induced by the EBM $P(x)$, where $Z=\sum_x P(x)$ is the normalization constant (partition function). Given an arbitrary EBM $P(x)$, %To solve this problem, \citet{opt-rl-arxiv-2019} propose a general approach for EBMs, which consists in fitting an autoregressive model (henceforth a ``policy'') $\pit$ to the distribution $p$, and then using $\pit$ as the sampler. They note that, with $\pi$ denoting an arbitrary distribution on $x$, and with   $\CE(p,\pi) \doteq - \EX{x \sim p} \log \pi(x)$ denoting cross-entropy between $p$ and $\pi$, the minimum in $\pi$ of $\CE(p,\pi)$, which is also the minimum of $\KL(p,\pi) = \CE(p,\pi) - H(p)$, is attained for $\pi = p$. This motivates their approach, in which they try to minimize the quantity 
DPG optimizes the loss function $\KL(p, \pit)$ with respect to the parameters $\theta$ of an autoregressive model $\pit$, 
\ptmd{a loss which is minimized for}
% which has a minimum at
$\pit=p$. 
% \citet{khalifa_2021} follow this approach, initializing $\pit = a$ and fine-tuning it according to the cross-entropy objective.
%
The KL-divergence minimization objective leads to a gradient estimate of the form:
\begin{align}
% \begin{split}
\nabla_\theta \KL(p, \pit) =& - \nabla_\theta \EX{x\sim p} \log \pit(x) \\
=& - \sum_x p(x) \nabla_\theta \log \pit(x) = - \frac{1}{Z}\sum_x P(x) \nabla_\theta \log \pit(x) \\
=& - \frac{1}{Z} \,\,\, \EX{x \sim \pit} \frac{P(x)}{\pit(x)} \nabla_\theta \log \pit(x).\label{eq:dpgon}
% \end{split}    
\end{align}

% \citet{opt-rl-arxiv-2019} propose two variants of their DPG algorithm to perform the optimisation: \DPGon, based on \eqref{eq:dpgon}, which samples directly from $\pit$, and \DPGoff, based on \eqref{eq:dpgoff}, which samples from a proposal distribution, $q$, that is periodically updated based on $\pit$:
% \begin{align}
%     \label{eq:dpgon}
%     \nabla_\theta \KL(p, \pit) &\propto \EX{x \sim \pit} \frac{P(x)}{\pit(x)} \nabla_\theta \log \pit(x) \\
%     \label{eq:dpgoff}
% &\propto \EX{x \sim q} \frac{P(x)}{q(x)}\nabla_\theta \log \pit(x),
% \end{align}
% where $-\frac{1}{Z}$ is the proportionality constant.

\begin{comment}
\subsection{Policy gradients}
Let's suppose that $R(x)$ is a ``reward'' associated with a sequence $x$. Then, the simplest policy gradient algorithm in reinforcement learning, namely, REINFORCE \citep{Williams92}, consists in finding the policy $\pit(x)$ that maximizes the average reward $\EX{x \sim \pit} R(x)$, and this leads, via the so-called ``log trick'', to a gradient ascent algorithm based on:
\begin{align}
  \label{eq:REINFORCE}
  \nabt \EX{\pit} R(x) = \EX{\pit} R(x) \nabt \log \pit(x),
\end{align}
which iteratively samples sequences $x$ from $\pit$ and update parameters by adding increments proportional to $R(x)\nabt \log \pit(x)$.
\end{comment}





==> RMvsDM NeurIPS 2022 Submission-5/sections/broader_impact.tex <==
\section{Broader impacts}
\label{section:Broader}
The focus area of this paper --- fine-tuning large language models --- is aligned with an important line of work on addressing the problem of social bias in large language models \citep{ShengCNP_LM_bias19,liang2021understanding}. As the training data for large language models consists mainly of crawled user-generated content, a number of factors (from crawling methodology to Internet participation inequalities and moderation practices) leads to an over-representation of certain viewpoints and voices exceeding their prevalence in the general population. This poses a risk of amplifying biases and harms through a language model perpetuating these voices \citep{Bender_parrots,blodgett-bias-survey,ShengCNP_LM_bias19,ethical_lm_deepmind,ethical_lm_deepmind2}. Numerous problems related to addressing data bias in language generation (e.g. controlling for gender distribution in generated texts) can be naturally posed as generative distributional control (GDC), the framework we focus our experiments on. The \emph{distributional} character of these data bias problems lies in the fact that desirable properties of generated texts are defined for a collection of samples, not only for individual samples. Our theoretical analyses of reward maximization and distribution matching approaches as well as our algorithmic improvements to the \GDC framework --- termed \GDCplus --- are therefore also a contribution to the problem of bias in language models. However, we need to be aware that \GDCplus, KL-control as well as controllable language generation techniques in general, can also be diverted to malicious uses such as spreading misinformation or generating harmful content.

==> RMvsDM NeurIPS 2022 Submission-5/sections/discussions.tex <==
Fine-tuning large language models has become an active area of research, due to its importance in adapting large language models to satisfy task-level preferences, or in combating their social risks such as “distributional” stereotyping~\citep{ethical_lm_deepmind, ethical_lm_deepmind2}.
\footnote{See Appendix \ref{section:Broader} for a discussion of broader impacts of large language models and controllable language generation.}
%
In this paper, we analyzed in depth the nuanced relation between two popular fine-tuning paradigms: RM and DM. We demonstrated that KL-control can be seen as \ptmd{a form of} DM and showed that while 
% some similarities between DPG and PG are superficial
\ptmd{DPG and PG have different goals,
%goals and techniques, 
some similarities}
(similar forms of gradient estimates despite different objectives) can be exploited. We used these insights to inform an extension of DPG, consisting in adding a baseline to reduce the variance of gradient estimates.

The connections we established suggest that despite fundamental differences between DPG and RL, some of the theoretical results and algorithmic techniques from RL can be adapted to a DM framework without losing their 
%theoretical 
\ptmd{formal}
guarantees. In this paper, we focus on variance reduction using baselines, but the space of possible enhancements is vast. Promising candidates include further reducing the variance using a learned value function \citep{conda_actor} and preventing detrimentally large policy updates by maintaining a trust region in the policy space -- akin to techniques such as TRPO \citep{schulman2015trust} and PPO \citep{schulman2017proximal}. \ptmd{Another future direction} could consist in analyzing the relation between explicit EBMs in DPG and implicit EBMs arising in KL-control and characterizing the space of EBMs 
% that can be represented in KL-control's objective. 
\ptmd{that could be reached through KL-control.}

% In this paper, we analyzed the nuanced relation between standard RL and the DPG family of algorithms and used these insights to inform an extension of DPG: adding a baseline. While RL is arguably a popular approach in finetuning language models to satisfy certain desiderata, alternatives enabled by DPG (such as \GDC and \GDCplus) enjoy a number of benefits. First,
%     % \item Modularity. DPG decouples specifying the EBM $P$ representing target constraints and approximating $P$ using an easy-to-sample-from policy. This is methodologically desirable because it forces an explicit and interpretable definition of the optimal solution and allows for posing\md{a bit heavy. Perhaps just ``poses''?} the second step as a well-defined problem of sampling from an EBM.\md{(See Latex source for full comment) I suggest removing the original sentence ``Instead,, RL ..,". The contrast is not with RL here, but with many EBM approaches that conflate training the EBM and sampling from it. Really, modularity is not a strong differentiator with RL, I think, and perhaps this item could go...} % Instead, RL merges the two steps which makes the actual properties of a maximum-reward solution hard to predict.
%     DPG is well-adapted to handle \emph{distributional constraints} (such as desired gender distribution) 
%     because it approximates the whole \emph{distribution} over samples as opposed to maximizing a reward $R(x)$ defined for a single sample $x$.
%     % \md{The focus here is in approximating the EBM, not on the moments, which come before the construction of the EBM. Our baseline technique is actually orthogonal to the moment aspect, so this could be misleading.}
%     %because its objective explicitly encourages matching \emph{moments} or expected values of generated samples through a target EBM. 
%  If it weren't for the limited capacity of the policy $\pit$, the expected reward objective would make it peak on a single sample associated with the highest possible reward.
%     The other benefit of the DPG framework is preventing 
%     undesired drift.
%     $p$ is guaranteed to be the policy closest to $a$ that satisfies all the constraints. Therefore, training $\pit$ using DPG avoids unnecessary drift from $a$ and maintains desirable properties of $a$ such as fluency and diversity. In contrast, $\pit$ trained with RL is prone to catastrophic forgetting of the desirable properties of $a$ and augmenting the reward with a KL penalty term (as in Ziegler) empirically results in unstable training.
% {\color{blue}In this study we provided a distributional Interpretation to KL-control approaches for fine-tuning LMs. We showed that this is equivalent to minimizing the reverse KL-divergence between an emergent EBM that takes a specific form. Unlike in ~\cite{khalifa_2021}, this underlying distribution is not defined explicitly. A promising future direction is how to manipulate this underlying distribution to conform to a target distribution of choice. We leave these questions to future work.}
% %%

% Nevertheless, RL enjoys a large number of theoretical results and algorithmic techniques. Despite fundamental differences between DPG and RL, at least some of these techniques can be adapted to a distributional setting without losing their theoretical guarantees. In this paper, we have focused on variance reduction using baselines, but the space of possible enhancements is vast. Promising candidates include further reducing the variance using a learned value function \citep{conda_actor} and preventing detrimentally large policy updates by maintaining a trust region in the policy space -- akin to techniques such as trust-region policy optimisation \citep{schulman2015trust} and proximal policy optimisation \citep{schulman2017proximal}. We leave the exploration of these possibilities to future work.


==> RMvsDM NeurIPS 2022 Submission-5/sections/experiments.tex <==
%%%%%%%%%%%%% Introduction to EBM forms %%%%%%%%%%%%%%%%%%%%% 
\subsection{Generation with Distributional Control}
% HE: added after rebuttal task consolidation

% examples for debiasing or classifier or topic control (add more citations)

%
We investigate the benefits of adding a baseline to the DPG algorithm, on the Generation with Distributional Control (GDC)~\citep{khalifa_2021} framework. %
GDC makes use of DPG to control the properties of pre-trained language models to satisfy certain constraints. 
%
In our experiments, follow target distribution form of  \citet{A-parshakova-etal-2019-global}, \citet{khalifa_2021} and \citet{pmlr-v162-korbak22a}, in which the EBM $P(x)$ is defined  so that its  normalized variant $p(x)$
matches a set of desired moments constraints on given features $\phi_i(x)$, while having a minimal KL divergence $\KL(p,a)$ from an original pretrained language model $a$, to avoid catastrophic forgetting. 

These constraints are expressed as conditions $\bar{\mu}_i = \EX{x \sim p} \phi_i(x)$, for $i \in \{1,\dots,n\}$, by which the moments (expectations) under the distribution $p$ of each feature $\phi_i(x)$ are required to take certain desired values $\bar{\mu}_i$. For instance, let $\phi_1(x) = 1$ iff the topic of $x$ is science and $\phi_2(x) = 1$ iff $x$ mentions a female person, then imposing moments $\bar{\mu}_1 = 1$ and $\bar{\mu}_2 = 0.5$ constrains the language model $p$ to only generate sequences about science, half of which mention females. $P(x)$ is uniquely determined by the following  form:\footnote{For a more precise formulation of this EBM, see \citep{khalifa_2021}.}
\begin{equation} 
    P(x) = a(x)e^{\sum_{i=1}^n \lambda_i \phi_i(x)}, \label{eq:target-EBM}
\end{equation}
where $\lambda_i$ terms control the moments $\mu_i$ of the associated features, which can be estimated through self-normalized importance sampling \citep{owen_chapter_importance_sampling_2013}; and then, to make the moments match the desired values, the $\lambda_i$ terms can be optimized through SGD~\citep{A-parshakova-etal-2019-global}.
%for controlled NLG / Khalifa

% for data efficient learning /  Parshakova
% In the case of \citet{A-parshakova-etal-2019-global} these moment constraints $\bar{\mu}_i$ are defined to match certain feature expectations of the training data, and the prior knowledge resulting from ``paying attention'' to these features leads to a more data-efficient learning.

%Here the $\lambda_i$'s are parameters ensuring moment matching, which can be estimated from a large sample from $a$ through self-normalized importance sampling \citep{A-parshakova-etal-2019-global,KimBengio2016,owen_chapter_importance_sampling_2013}.
%
% The equation for snis is incomplete (sum over i). I think we can avoid entering into this aspect here.
% by minimizing the mean-square error between desired moments $\bar{\mu}_i$ and estimated moments $\hat{\mu}_i = \frac{\sum_n^N \exp{(\lambda_i \phi_i(x))} \phi_i(x)}{\sum_n^N \exp{(\lambda_i \phi_i(x))}}$, based on $N$ samples obtained through self-normalized importance sampling \citep{KimBengio2016,A-parshakova-etal-2019-global}.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% Experimental Setup %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experimental setup}\label{subsec:exp_setup}

We evaluate our method on an array of 10 controlled text generation tasks. For each, given a pre-trained language model $a(x)$, and a set of constraints, the objective of each fine-tuning method is to obtain a fine-tuned language model $\pit$ that satisfies the imposed constraints while deviating as minimally as possible from the original language model $a(x)$. 

Constraints are defined as a set of binary features $\{\phi_i\}$ and their corresponding desired percentages (moments) $\{\bar{\mu}_i\}$ within the generations of the target language model.
%
% \vspace{-5px}
% \paragraph{Tasks}
% We evaluate GDC, GDC\texttt{++} and the two baselines on \textbf{10 tasks}, 
% which we construct through sets of moment constraints $\{\bar{\mu}_i\}$ for binary features $\{\phi_i\}$. 
Based on the value of the moment constraints these 10 tasks are divided into 6 tasks of pointwise constraints (for which  $\bar{\mu}_i = 1$), 2 tasks of distributional constraints ($0 < \bar{\mu}_i < 1$) and 2 tasks of mixed type constraints (hybrid):
\vspace{-0.1cm}
\begin{enumerate}[label=(\alph*)]
    \itemsep0em 
    \item Single-word constraints, where $\phi(x) = 1$ iff the a given word appears in the sequence $x$. We experiment with frequent words (task 1: ``amazing'', original frequency: $10^{-4}$) and (task 2: ``WikiLeaks'', original frequency: $10^{-5}$) rare words,
    \item Wordlist constraints, where $\phi(x) = 1$ iff $x$ contains at least one word from a given list. We consider lists of word associated with politics (task 3) and science (task 4) published by \citet{plug_and_play_20},
    \item Sentiment classifier constraints, where $\phi(x) = 1$ if $x$ is classified as positive (task 5), or negative (task 6) by a pre-trained classifier published by \citet{plug_and_play_20}.
    \setcounter{enumi}{3}
    \item A single distributional constraint where $\phi(x) = 1$ iff $x$ contains a female figure mention, and $\bar{\mu} = 0.5$ (task 8),
   \item A set of four distributional constraints: $\phi_i(x) = 1$ iff $x$ contains at least one of the words in the ``science", ``art", ``sports" and ``business" wordlists (compiled by \citet{plug_and_play_20}), respectively. For each $i$, $\bar{\mu}_i = 0.25$ (task 8),
    \item Hybrid constraints where $\phi_1(x) = 1$ iff $x$ contains more female than male pronouns, $\bar{\mu}_1 = 0.5$ and $\phi_2(x) = 1$ iff $x$ contains at least one of the words from the ``sports" wordlist (task 9) or ``politics'' wordlist, $\bar{\mu}_2(x) = 1$ (task 10).
\end{enumerate}
\vspace{-0.2cm}
\paragraph{Methods}
We modify the GDC framework~\cite{khalifa_2021}, namely its KL-DPG algorithm, to include a baseline as shown in \Algref{al:KL-adaptive-DPG-baseline}. We refer to this method as \textbf{GDC\texttt{++}}. 
%
In addition to comparing \textbf{GDC\texttt{++}} with \textbf{GDC}
%, for tasks for which the comparison is meaningful (i.e. for ``pointwise constraints", see below), 
we compare with two reward maximization baselines: \textbf{Reinforce} \citep{Williams92Reinforce} and \textbf{Ziegler} \citep{Ziegler19}. Reinforce tries to maximize the expected reward $\E_{x \sim \pit} R(x)$, where $R(x) =1$ if and only if the pointwise constraints are met. Ziegler instantiates the KL-control approach: its objective includes a KL penalty term for departures from $a$.
%
Following~\citep{khalifa_2021}, for hybrid and distributional constraints (tasks 8-10) we compare only GDC and GDC\texttt{++} because the RM objective of Ziegler and Reinforce is not equipped to handle them. 

%%%% EVAL METRICS %%%%
\vspace{-5px}
\paragraph{Metrics} 
We report the following metrics at each validation step over batches of samples from $\pit$:
\vspace{-0.3cm}
\begin{enumerate}
    \itemsep0em 
    \item $\E_{x \sim \pit} \phi_i(x)$, measuring the ability to reach the target moment of the $i$-th feature. 
    \item $\KL(p, \pit)$, the forward KL divergence from the optimal target distribution $p$,\footnote{See Appendix \ref{detailed-metrics} for a detailed description of how $\KL(p, \pit)$ is computed.}
    % , this is a proxy to both fluency and satisfaction of control conditions. 
    \item $\KL(\pit, a)$, the reverse KL divergence from the original pretrained language model $a$. 
    \item Distinct-n score, a measure of text diversity in terms of the frequency of repetitions within a single sample $x$, proposed by \citep{li-etal-2016-diversity}. 
    % Low values of Distinct-n scores indicate high number of repetitions within a single sequence which is a signal of \textit{degeneration} due to \emph{catastrophic forgetting}.
    \item Self-BLEU-n, a measure of text diversity on a distributional level \emph{across} samples proposed by \citep{texygen-ZhuLZGZWY18}, ensuring that policies don't converge into limited number of sequences that satisfy the imposed constraints~\cite{GAN_short}.
\end{enumerate}
\vspace{-10px}
\paragraph{Training details}
For tasks 1-6, we use a pre-trained GPT-2 small with 117M parameters \citep{radford2019language} as the original language model $a$. For tasks 7-10, $a$ is the same pre-trained model additionally fine-tuned on the WikiBio~\citep{DBLP:conf/emnlp/LebretGA16} dataset. See Appendix \ref{appendix:Hyperparameters} for more details. The code for all the experiments presented in the paper will be available at \href{https://github.com/naver/gdc}{github.com/naver/gdc}.

%%%%%%%%%%%%%%%%%%%
%%%%% Results %%%%%
%%%%%%%%%%%%%%%%%%%
% \input{figures/table_pointwise_dist_experiments}
\subsection{Results}
\label{subsec:general_results}
We present the evolution of our metrics through training epochs in Figure \ref{fig:pointwise-compare-methods-metrics} (aggregated over tasks 1-6) and Figure \ref{fig:distributional-compare-methods-metrics} in the Appendix (aggregated over tasks 7-10). Results for each task are presented separately on Figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} in the Appendix.

Consistent with prior work~\citep{khalifa_2021,pmlr-v162-korbak22a}, we observe that Reinforce is able to quickly achieve high levels of constraint satisfaction, but at the cost of large deviations from $a$, which translates into significantly decreased diversity of generated samples (in terms of Self-BLEU-5 and Distinct-1). The KL penalty term in Ziegler imposes an upper bound on deviation from $a$ but the deviation is still significant enough to result in a drop in diversity. Moreover, we have observed Ziegler's objective to result in very unstable training. 

\GDC and \GDCplus are the only fine-tuning methods that address constraint satisfaction based on a clear formal objective, i.e. reducing the divergence from $p$. The approach translates into significantly smaller deviations from $a$ and maintaining diversity within and across samples. The addition of a baseline indeed reduces the variance. We analyze that extensively in Appendix \ref{subsec:effectOnVarReduc} while here focusing on the downstream effects of variance reduction. One is that $\pit$ is now able to compound staying closer to $p$ and $a$ \emph{at the same time}, while achieving slightly better constraint satisfaction. We have also observed that baseline stabilizes training, leading to smoother curves.\footnote{The interested reader can compare the large fluctuations of the Ziegler objective to more stable training curves of \hbox{\GDC,} and even more of \GDCplus, in the disaggregated curves in Figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} of the Appendix.} 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%% Plots of RESULTS %%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{figures/table_bsz_experiments}
\begin{figure*}[t]
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=\linewidth]{figures/pointwise-compare-methods-metrics.pdf} 
    \caption{\small{Evaluation metrics:  $\KL(p, \pi_{\theta})$ ($\downarrow$ better), $\mathbb{E}_{\pit} \phi(x)$ ($\uparrow$ better), $\KL(\pi_{\theta}, a)$ ($\downarrow$ better), Self-BLEU-5 ($\downarrow$ better), and Distinct-1 ($\uparrow$ better) aggregated over 6 pointwise constraints experiments (tasks 1-6) for policies obtained from GDC\texttt{++}, GDC, Ziegler and Reinforce. See Figure~\ref{fig:distributional-compare-methods-metrics} for aggregated distributional constraints experiments. In the Appendix Figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} and Table~\ref{tab:all_experiments_results} contain individual view and final results of each run.}}
    \label{fig:pointwise-compare-methods-metrics}
\end{figure*}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{.51\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/gdc_batch_size_point.pdf} 
    \caption{\small{Task 1: a pointwise constraint}}
    \label{fig:gdc_batch_size_point}
    \end{subfigure}%
    %
    \begin{subfigure}[t]{.51\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/gdc_batch_size_dist.pdf} 
    \caption{\small{Task 8: a set of distributional constraints; $\bar{\mu}_i = 0.25$}}
    \label{fig:batch_size_dist}
    \end{subfigure}

    \caption{\small{
    $\mathbb{E}_{\pit} \phi(x)$ or $\hat{\mu}$ per constraint ($\uparrow$ better) and $\KL(p, \pi_{\theta})$ ($\downarrow$ better) as a function of the number of samples reported for task 1 (a) and task 8 (b). We report the number of samples (i.e. the number of epochs times the batch size) for a fair comparison of convergence speed. \emph{\GDCplus is consistently superior across all batch sizes in terms of convergence and constraint satisfaction}. The effect is more conspicuous with small batch sizes. 
    % For instance, with batch size 256 the baseline prevents the policy from catastrophically diverging from $p$. 
    Batch sizes 512 and 2014 are greyed out for clarity. 
    }}
    \label{fig:bsz}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% BATCH SIZE analysis %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-5px}
\subsection{The effect of baseline across batch sizes}
\label{subsec:bsz_exps}
We expect that reducing gradient estimates variance can allow to train with lower batch sizes, performing gradient updates on estimates based on smaller batch sizes can increase the sample efficiency. 
%
To test this, we rerun tasks 1 (a pointwise constraint on the word ``amazing") and 8 ( distributional constraints on topics) with four batch sizes (256, 512, 1024, 2048). 
%
Figures \ref{fig:gdc_batch_size_point} and \ref{fig:batch_size_dist} show the benefits of adding a baseline --- higher constraint satisfaction, lower divergence from $p$, more stable training --- and is especially evident with lower batch sizes. 
For instance, with batch size 256, \GDCplus obtains a significantly higher constraint satisfaction rate and lower divergence from $p$.

Furthermore, stable training with smaller batch sizes translates into better sample efficiency. For instance, in task 1 (Figure \ref{fig:gdc_batch_size_point}), \GDCplus with batch size 256 needs 1M samples to achieve $\E_{x \sim \pit} \phi(x) = 0.5$ while \GDCplus with batch size 2048 needs 4M. In contrast, \GDC with batch size 256 does not achieve $\E_{x \sim \pit} \phi(x) = 0.5$ at all, confirming the importance of adding the baseline.

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/gdc_batch_size_dist.pdf} 
%     \caption{\small{$\hat{\mu}$ (one per constraint; $\uparrow$ better) and $\KL(p, \pit)$ ($\downarrow$ better) as a function of the number of samples used in training to satisfy a set of distributional constraint (task 8; target: ). We report the number of samples (i.e. the number of epochs times the batch size) for a fair comparison of convergence speed. Batch sizes 512 and 1024 are greyed out for clarity. Again we can see consistent improvement across all batch sizes.}}
%     \label{fig:batch_size_dist}
% \end{figure*}


==> RMvsDM NeurIPS 2022 Submission-5/sections/intro.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[draft=false,width=\linewidth]{figures/DPG++.pdf} 
%     \caption{\small{
%     In this study we make connection between two popular paradigms for fine-tuning sequence generation models according to preferences \emph{Reward Maximization} (RM) and \emph{Distribution Matching} (DM).
%     }}
%     \label{fig:intro}
%     \vspace{-10px}
% \end{wrapfigure}


Pre-trained language models \citep{devlin-etal-2019-bert,radford2019language} are changing the landscape of Machine Learning research and practice. 
%
Due to their strong generative capabilities many studies have found it sufficient to ``nudge'' these models to conform to global preferences defined over the generated sequences instead of training from scratch using annotated data. These preferences could include
%
topic and sentiment~\citep{plug_and_play_20}, valid musical notes and molecular structures~\citep{KL_Jaques17}, code compilability~\citep{korbak2021code}, reducing distributional biases~\citep{khalifa_2021, ethical_lm_deepmind}, evaluation metrics for Machine Translation and Summarization~\citep{seq_lvl_train_RanzatoCAZ15,bahdanau_actor-critic_2016}, or direct human feedback~\citep{Ziegler19,ziegler_summarize2021}.
%
This large body of studies is driven by two different paradigms: \emph{Reward Maximization} (RM) and \emph{Distribution Matching} (DM).

% \begin{wrapfigure}{c}{\textwidth}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/RMvsDM_fig.pdf} 
    \caption{\small{
    In this study we make a connection between two popular paradigms for aligning language models to human preferences: Reward maximization (RM) and Distribution matching (DM).
    }}
    \label{fig:intro}
\end{figure}
% \end{wrapfigure}

\paragraph{Reward Maximization}
RM intuitively nudge\ptmdII{s} pre-trained models towards \ptmdII{certain} preferences by providing global sequence-level rewards when the model generates outputs that satisfy desired features.
For instance, if the model is producing toxic content, we can apply Reinforcement Learning (RL) techniques to discourage it from producing similar content. 
%
However, naively applying RL yields \ptmdII{a} model that \ptmdII{can} undergo \emph{catastrophic forgetting} of its original distribution.
For example, it can degenerate into producing a single nonsensical but at least nontoxic sequence. 
%
% Early enough, limitations of maximisation vanilla rewards were exposed. 
Although several studies have considered hand-crafting general rewards to ensure desirable features like fluency~\citep{LiuLSNCP16,RL_TambwekarDMMHR19}, coming up with complete or perfect rewards is highly non-trivial~\citep{Wu_googleMT16,VedantamZP15}. This has sparked a wide discussion on the overall effectiveness of RM for some tasks such as machine translation~\citep{Choshen20WeaknessRL,KiegelandK21}.%
\fmdII{The figure is nice, but small print is a bit pale, perhaps make the color darker.}

% KL control 
\paragraph{Reward Maximization with KL-Control}
To tackle the aforementioned issues of ``catastrophic forgetting'', several studies, still under an RM paradigm, have considered incorporating a distributional term inside the reward to be maximized. In particular~\citet{Jaques-2017,KL_jaquesK19} and \citet{Ziegler19} or more recently \citet{ziegler_summarize2021}, \citet{Ouyang}, \citet{bai2022training} and \citet{redteaming} have applied variations of KL-control~\citep{todorov,kappen2012optimal} which adds a penalty term to the reward term so that the resulting policy does not deviate too much from the original one in terms of KL-divergence. The overall objective with the KL-penalty is maximized using an RL algorithm of choice including: PPO~\citep{PPO} as in \cite{Ziegler19} or \cite{bai2022training} or Q-learning~\citep{MnihKSGAWR13} as in~\cite{Jaques-2017}.
%
Adding this \emph{distributional} KL-penalty to the reward raises some important questions:
% todo: perhaps remove since not so important
% Since the reward -as we show later- now becomes parametric i.e. dependent on the policy being optimized, is it theoretically principled to maximize this parametric reward using standard policy gradient or other RL algorithms that follows the same derivation? 
%
What effect does it have on the shape of the optimal policy? Does this new objective have any interpretation from a distributional perspective?
%and since the distributional aspect i.e. the KL divergence from the pre-trained model, is an important aspect of this RM process in general, 
%%

\paragraph{Distribution Matching}
A different \ptmd{recent} paradigm for fine-tuning language models to satisfy downstream preferences formulates the problem as Distribution Matching (DM).
%
This paradigm consists of two steps: first a target distribution incorporating the desired preferences is defined as an Energy-Based Model~\citep{lecun_tutorial_2006}.
% (a probability distribution that doesn't have to be normalized)
%
Then the forward KL divergence is minimized between this target distribution and an auto-regressive policy using a family of algorithms referred to as Distributional Policy Gradients (DPG)~\citep{opt-rl-arxiv-2019,khalifa_2021,korbak2021code,pmlr-v162-korbak22a}. 
%
This approach capitalizes on the flexibility of EBMs in specifying the target distribution. For example, the EBM can be defined so that it conforms to all downstream preferences while its corresponding normalized distribution has a minimal KL divergence from the original, pre-trained language model, therefore tackling the problem of ``catastrophic forgetting''~\citep{khalifa_2021}.
% todo: summarize next paragraph:
Interestingly, this DM paradigm can also deal with \emph{distributional} preferences, for instance, for de-biasing language models by specifying that the generated sequences should be gender-balanced, i.e. that 50\% of generations contain female mentions. Such distributional constraints cannot be defined in the RM paradigm where a reward is calculated for a single sequence. 
% DPG is inspired by vanilla Policy Gradients~\citep{sutton_policy_gradients} leading to superficially similar gradients, yet, the exact relation of DPG to Policy Gradients in standard RL remains poorly understood.\ftk{This sentence doesn't really connect with what's before and after. I'd remove?}

% paragraph of conclusion questions and cliff hangers to engage reader
We can notice the promises and limitations of these two paradigms for fine-tuning language models. RM approaches are equipped with an arsenal of RL algorithms and optimization techniques that \ptmd{can}
be efficient in reward maximization, however they lack the distributional aspect to avoid catastrophic forgetting and impose distributional  preferences over LMs. 
% \ptmd{controlling distributional properties of LMs.}
DM approaches are suited to tackle those limitations,
however, the family of DPG algorithms % typically used in DM 
\ptmd{currently used}
is not as rich as its RL counterpart.
%
% MD 31/07/2022 BEGIN of Commenting out this section 
% So far, the connections between these two seemingly distinct paradigms have not been thoroughly explored. 
% % If we establish those 
% \ptmd{By establishing such connections we might}
% import ideas from one approach to the other. 
% %In this paper, we give an answer to these %aforementioned 
% %questions, showing that there is indeed a connection between RM and DM, which we leverage to import variance reduction techniques from RM into DM. 
% \ptmd{This is our goal in this paper, detailing the nuanced connections and applying them to a case-study in variance reduction.}
% Overall, our contributions %in this study
% are the following: 
% \vspace{-5px}
% % \begin{itemize}[leftmargin=*]
% %     \itemsep0em 
% %     \item  We \ptmd{untangle}
% %     % demystify
% %     \fmd{(4-10) demystify: maybe not the right word: this supposes that there are established beliefs about DPG in the community... Would use something like ``disentangle'', ``clear up''...} 
% %     the connections between the RM and DM paradigms for fine-tuning LMs. We provide a detailed comparison of the family of DPG algorithms with the Policy Gradients of standard RL, and provide an interpretation of KL-control techniques from a distribution matching perspective,
% %     %
% %     \item We exploit these connections to theoretically justify applying \emph{baselines} --- a variance reduction technique from RL --- to DPG and derive of a particular choice of a baseline,
% %     %
% %     \item We empirically validate the benefits of adding a baseline on an array of controllable language generation tasks such as constraining topic, sentiment, and gender distributions in texts sampled from a language model and show that adding baselines leads to superior performance in terms of constraint satisfaction, stability on small batch sizes and sample efficiency.\fmd{(4-10) MORE IMPORTANT: Wondering whether it would not be more strategic to make two bullets out of the first bullet and one bullet out of the second and third bullets.} 
% %     %
% %     % Looking only at KL, it appears that the proposed method (GDC++) can achieve in 2.5 million samples what GDC can achieve in 5 million.
% % \end{itemize}
% %
% \begin{itemize}[leftmargin=15px]
%     \itemsep0.2em 
%     \item  We reveal connections between the RM and DM paradigms through a detailed comparison between the family of DPG algorithms with Policy Gradients (Table \ref{tab:comparison_DPGvsPG}).
%     %
%     \item We introduce an interpretation of KL-control techniques from a distribution matching perspective, placing such techniques at an intermediate place between RM and DM (Theorem \ref{theorem_kl}).
%     %
%     \item We show how these connections can enable cross-pollination between the two perspectives by applying \emph{baselines} --- a variance reduction technique from RL --- to DPG and derive a particular choice of a baseline (Facts \ref{dpgon_baseline_unbiased} and \ref{dpgoff_baseline_unbiased}). On an array of controllable language generation experiments, % about constraining topic, sentiment, and gender distributions over a pre-trained language model, 
%     we show that adding baselines leads to superior performance on constraint satisfaction (Figure \ref{fig:pointwise-compare-methods-metrics}), stability on small batch sizes, and sample efficiency (Figure \ref{fig:bsz}). 
%     %
%     % Looking only at KL, it appears that the proposed method (GDC++) can achieve in 2.5 million samples what GDC can achieve in 5 million.
% \end{itemize}
% MD 31/07/2022 END of Commenting out this section 


\ptmdAR{While the connections between these two seemingly distinct paradigms have been noted \citep{opt-rl-arxiv-2019,rl_kl_penalties}, they have not been explored in detail. 
Clarifying such connections might help import ideas from one approach to the other. 
This is our goal in this paper, detailing the nuanced connections and applying them to a case-study in variance reduction.}
Overall, our contributions are the following: 
\begin{itemize}[leftmargin=15px]
    \itemsep0.2em 
    \item  \ptmdAR{We clarify relations between the RM and DM paradigms through a detailed comparison between the family of DPG algorithms and Policy Gradients (Table \ref{tab:comparison_DPGvsPG}), stressing the differences between \emph{parametric} and \emph{non-parametric} rewards that are important in this regard.}  
    %
    \item We introduce an interpretation of KL-control techniques from a distribution matching perspective, placing such techniques at an intermediate place between RM and DM (Theorem \ref{theorem_kl}).
    %
    \item We show how these connections can enable cross-pollination between the two perspectives by applying \emph{baselines} --- a variance reduction technique from RL --- to DPG and derive a particular choice of a baseline (Facts \ref{dpgon_baseline_unbiased} and \ref{dpgoff_baseline_unbiased}). On an array of controllable language generation experiments, 
    we show that adding baselines leads to superior performance on constraint satisfaction (Figure \ref{fig:pointwise-compare-methods-metrics}), stability on small batch sizes, and sample efficiency (Figure \ref{fig:bsz}). 
\end{itemize}

==> RMvsDM NeurIPS 2022 Submission-5/sections/klcontrol.tex <==
%% optimizing the PG term is not necessary 
Adding a KL-penalty term to the reward (as in the case of KL-control)\fmd{Harmonise KL-control vs KL control.} leads to a parametric reward. However, due to the particular form of its objective, the RG-term actually \emph{vanishes},\footnote{This is because $\E_\pit \nabt \Rtz(x) = -\beta\, \E_\pit \nabt \log \pit(x) = 0$, via the 
% often used 
identity $\E_\pit \nabt \log \pit(x) = \sum_x \pit(x) \nabt \log \pit(x) = \sum_x \nabt \pit(x) = \nabt \sum_x \pit(x) = 0$.}
leaving only the PG-term $\E_{x \sim \pit} \Rtz(x) \nabt \log \pit(x)$ and simplifying the tuning procedure to a standard Policy Gradient.
%%%%% 
While this algorithm falls under the RM paradigm, here we argue that is its nature is multifaceted, and explore deeper connections with the DM paradigm. 
More precisely, the maximization of reward with the KL penalty term is equivalent to a distributional matching with an underlying emergent sequential EBM, a remark that already reveals some similarities with DPG.\footnote{The optimal policy $p_z$ is briefly mentioned in \citep{Ziegler19} without reference or derivation. The proof, which 
%we believe to clarify important underlying connections
\ptgk{reveals a connection to the reverse KL divergence from $\pit$},
is ours.}
% Actually, the distribution 
% % $p_z$ 
% that obtains maximal expected reward $\Rtz(x)$ can be defined by the following sequential EBM $P_z$:
% \begin{equation}
%     p_z(x)  = \frac{1}{Z} \; P_z(x) = \frac{1}{Z} \; a(x)e^{r(x)/\beta}. \label{eq:Ziegler_optimal}
% \end{equation}


\begin{theorem}
\label{theorem_kl}
Consider the following EBM:
\begin{equation}
   P_z(x) = a(x)e^{r(x)/\beta} \label{eq:Ziegler_optimal}
\end{equation}
and let $p_z$ be the normalized distribution $p_z(x)  = \frac{1}{Z}\;  P_z(x)$, with $Z=\sum_x P_z(x)$. Then: 
\begin{enumerate}[itemsep=0pt, label=(\roman*)]
    %\itemsep0em
    \item $\argmax_\pit \E_{x \sim \pit} \Rtz(x) = \argmin_\pit \KL(\pit, p_z)$;
    \item $\argmax_{\pi \in \mathcal{D}(X)} \E_{x \sim \pi} \Rpiz(x) = p_z$, 
    where $\mathcal{D}(X)$ is the family of all distributions over $X$, and $\Rpiz(x) \doteq r(x) - \beta \log \frac{\pi(x)}{a(x)}$.
\end{enumerate}
%the normalized distribution $p_z(x)  = \frac{1}{Z}\; P_z(x)$ maximizes $J(\pit) = \E_{x \sim \pit} \Rtz(x)$.
%its normalized distribution, $p_z(x)  = \frac{1}{Z} \; P_z(x)$, with $Z = \sum_x P_z(x)$, is, among all possible distributions, the one  
%that obtains maximal expected reward $\Rtz(x)$.
\end{theorem}
\vspace{-5px}
\begin{proof}
A simple way to prove  this is to notice that the expectation of the reward $\Rtz$ %\eqref{eq:Rtz}
has a monotonically decreasing relationship with the \emph{reverse} KL divergence between $\pit$ and $p_z$:
% The monotonically decreasing relation between $\KL(\pi, p_z)$ and $J_\text{z}(\pi)$ results from the following derivation:
%\begin{small}
\begin{align*}
        \KL(\pit, p_z) &= \E_{x \sim \pit} \log \frac{\pit(x)}{p_z(x)}
    = \E_{x \sim \pit} \Big[\log \pit(x) - \log \frac{1}{Z} a(x)e^{r(x)/\beta}\Big] \\
    &= \log Z - \frac{1}{\beta}\, \E_{x \sim \pit} \Big[r(x) -\beta \log \frac{\pit(x)}{a(x)}  \Big] = \log Z - \frac{1}{\beta}\, \E_{x \sim \pit} \Rtz(x), \numberthis \label{eq:klrmax}
\end{align*}
so that the $\argmin_{\pi_\theta} \KL(\pit, p_z)$ coincides with the $\argmax_{\pi_\theta} \E_{x \sim \pit} \Rtz(x)$, proving (i). On the other hand, $\argmin_{\pi \in \mathcal{D}(X)} \KL(\pi, p_z)$, which also corresponds to $\argmax_{\pi \in \mathcal{D}(X)} \E_{x \sim \pi} \Rpiz$ because of (i) applied to a family $\pi_{\theta'}$ covering $\mathcal{D}(X)$ in full, is just $p_z$, concluding the proof.
%Provided that the family of distributions $\pit$ is large enough to cover all distributions over $X$, $\argmin_{\pi_\theta} \KL(\pit, p_z)$ is just $p_z$, which concludes the proof.
\end{proof}
% \vspace{-5px}
% {\color{orange}
% Overall, we can conclude that, the addition of the distributional term (KL-penalty) to the reward does indeed provide a DM interpretation, namely in terms of minimizing the reverse KL divergence with an emergent underlying distribution $p_{z}(x)$. It is important to note that $p_{z}(x)$ can not be explicitly defined to any distribution of choice (e.g. the one that balances the gender distribution of a language model). Instead it is implicitly defined on the specific form above in equation~\eqref{eq:Ziegler_optimal}. Which shows that the KL-control approaches are limited in their distributional expressivity, compared to the family of DPG algorithms which are designed to perform DM on any explicit distribution of choice.
Overall, we can conclude that the addition of the distributional term (KL-penalty) to the reward does indeed provide a DM interpretation, namely in terms of minimizing the reverse KL divergence with an emergent underlying distribution $p_{z}(x)$. We note that $p_{z}(x)$ 
%is not explicitly defined as any EBM of choice 
\ptmd{does not correspond to a free and explicit choice of EBM} 
(e.g. one that balances the gender and topic distributions of a language model). Instead equation~\eqref{eq:Ziegler_optimal} 
% has a limited form
appears in a restrictive format, which is
implicitly defined by the reward $\Rtz$, along with a $\beta$ hyperparameter without a clear meaning. By contrast, the DPG algorithms are designed to perform DM on any EBM specification, corresponding to an explicit distributional objective.
% }

==> RMvsDM NeurIPS 2022 Submission-5/sections/oldies (but goodies?)/intro.tex <==
%TODO: move somewhere else
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure1.pdf} 
    \caption{\small{
    Training trends of the Distributional Policy Gradient algorithm (DPG) for approximating Sequential Energy-Based Models. The addition of a \textit{baseline} reduces the variance of gradient estimates (left), leading to better convergence (right). 
    }}
    \label{fig:intro}
\end{wrapfigure}


With the advent of Large Language Models (LLMs), there has been a growing need for learning methods that require less data and for techniques to control the properties of the generated sequences, such as removing bias or harmful expressions~\citep{Bender_parrots,Bommasani:etal:2021}.
Sequential energy-based models (EBMs) have been recently recognized as a theoretically principled way of tackling these challenges by either injecting prior knowledge into these models \citep{A-parshakova-etal-2019-global,Deng2020Residual} or by imposing constraints upon them \citep{Naskar2020EnergyBasedRI,he-etal-2021-joint,khalifa_2021}. 
Describing their functioning in few words, they can represent constraints or prior knowledge about relevant features as sequence-level functions that can be combined with the model's own scores to describe an unnormalized distribution $P(x)$ over the space of possible sequences $x$.
However, whereas it is often simple to sample from an autoregressive language model, there is no obvious way to obtain samples from Sequential EBMs.

Distributional Policy Gradients (DPG)~\citep{opt-rl-arxiv-2019} are a family of learning algorithms that learn an autoregressive policy that approximates the probability distribution $p(x) = P(x)/Z$ induced by the EBM. 
In this way, it is possible to sample from the EBM by sampling from the autoregressive policy.
DPG was inspired by Policy Gradients (PG)~\citep{Williams92Reinforce}, a well-known technique in Reinforcement Learning. 
However, the extent to which the two approaches relate has not yet been thoroughly analyzed.
Establishing a formal connection between the two methods can have important consequences because if we succeed at it, DPG could benefit from a vast wealth of knowledge about PG that has been accumulated for over the past 30 years of research in RL.
In turn, this connection would directly impact all techniques built upon DPG.

In this paper, we make a detailed account of how the concept of reward, central to RL, translates into the DPG framework.
As a consequence, we can import well-established variance reduction techniques such as \emph{baselines}. 
We apply these insights to improve the GDC (Generation with Distributional Control) algorithm, a particular instantiation of DPG proposed by \citet{khalifa_2021} to \emph{control} language models.
This method is unique in allowing to define \emph{distributional} constraints on the language model while preventing \emph{catastrophic forgetting} of the original language model distribution.
Thanks to these properties, it can be applied to \emph{debiasing} the probability distributions of sequences containing mentions of different genders, among other usages such as constraining the topic or sentiment distribution.
Our results show a significant decrease in the variance of gradient estimates, thus obtaining improved constraint satisfaction, stability and sample efficiency.
Moreover, the improved algorithm has a much higher sample efficiency.
It can, for example, reach the performance that GDC achieves after $5$ million examples in half as many.


% Sequential energy-based models (EBMs) have been recently recognized as a theoretically principled way of injecting prior knowledge into autoregressive language models \citep{A-parshakova-etal-2019-global,Deng2020Residual} or of imposing constraints upon them \citep{Naskar2020EnergyBasedRI,he-etal-2021-joint,khalifa_2021}. 

% Sequential EBMs represent constraints or prior knowledge of relevant features as sequence-level functions that are combined with the scores of a language model to construct an unnormalized probability distribution $P(x)$.
% However, it is not clear how to obtain samples from the associated probability distribution $p(x) = P(x)/Z$ where $Z$ is the partition function.

%
% todo add more applications from ACL anthology papers
% EBM Cloze models~\cite{ClarkLLM20} 
%
% In this context, a sequential EBM $P(x) = a(x) b(x)$ is an unnormalized probability distribution over sequences $x$ which combines the probability scores of a base autoregressive model $a(x)$ with a nonnegative ``modifier'' $b(x)$ to express a preference towards certain sequences $x$. For instance, Generative Distributional Control or GDC~\citet{khalifa_2021} poses controllable language generation as a constraint satisfaction problem in which a pretrained language model is fine-tuned to approximate a target language model that fully satisfies some predefined constraints leading to an exponential expression for $b(x)$. Similarly, Global Autoregressive Models \citep{A-parshakova-etal-2019-global} and Residual EBMs \citep{Deng_EBM_20} enable data-efficient learning by augmenting an autoregressive language model with prior knowledge about its training data, expressed as preference towards certain sequences. In yet another line of work, \citet{Naskar2020EnergyBasedRI} augment a machine translation model $a$ with an energy-based reranker $b$: while $a$ was trained with maximum likelihood, $b$ prefers translations with high BLEU scores. In each case, $b(x)$ is flexible enough to represents requirements that couldn't be easily integrated in the training objective for $a$.

% The flexibility comes at a price: $P$ cannot be easily sampled from. This can be circumvented by training a second autoregressive model $\pit$ to approximate the normalized distribution $p$ associated with the target EBM $P(x)$. A family of algorithms, Distributional Policy Gradients (DPG), inspired by reinforcement learning (RL), was recently proposed as a solution to this approximation problem \citep{opt-rl-arxiv-2019,khalifa_2021}. Yet, the exact relation of DPG to Policy Gradients in standard RL remains poorly understood. In this work, we start by revisiting the motivations behind DPG and expose both fruitful connections but also important differences between DPG and standard RL. While RL typically tries to find a policy $\pit$ that maximizes the expected reward $\E_{x \sim \pit} R(x)$, DPG minimizes the distributional discrepancy (measured through cross-entropy) between an auto-regressive policy $\pit$ and the target EBM $P$. These two objectives imply similar functional forms of policy gradient estimates yet produce vastly different policies.

%  The connections we find between DPG and standard RL allow us to derive a DPG variant of \emph{baselines}, a popular variance reduction technique in standard RL \cite{suttonphd,williams1987}. In particular, we argue for a remarkably simple form of baseline: $Z = \sum_x P(x)$, the normalizing constant (partition function) associated with $P$. We empirically validate the benefits of adding such a baseline on an array of controllable language generation tasks such as constraining the topic, sentiment, or gender distribution of texts sampled from $\pit$. We observe a significant decrease in the variance of gradient estimates which translates into improved constraint satisfaction, stability and sample efficiency.
 
To summarize, the main contributions of the paper are:
% \vspace{-0.4cm}
\begin{itemize}
    \itemsep0em 
    \item A detailed comparison of the family of DPG algorithms with the policy gradients of standard RL,
    \item A theoretical justification for applying baselines --- a variance reduction technique from RL --- to DPG and a derivation of a particular choice of a baseline,
    \item An extensive empirical evaluation of the proposed algorithm --- DPG with baseline --- on controllable language generation tasks following the GDC approach, which results in more stable learning and higher sample efficiency.
\end{itemize}


%% some intro
% XXXX \\
% %%%
% a Sequential Energy based models - EBM over sequences. 
% %%%%
% In order to approximate a sequential EBM into an auto-regressive policy a recent class of algorithms referred to as Distributional Policy Gradients~\cite{A-parshakova-etal-2019-global} and its adaptive variants \cite{khalifa_2021} has been introduced.
% %
% This class of algorithms is intrinsically different in its objective to Standard Reinforcement Learning ones. It aims at minimizing the cross entropy objective between an auto-regressive policy $\pit$ and the underlying target distribution $p$ represented by the sequential EBM. While Standard Reinforcement Learning typically try finding a policy $\pit$ that maximize the expected reward $E_{\pit} R(x)$.
%


% Overall, our main contributions can be summarized as:
% \begin{itemize}
%     \item We revisit theory proposed in \cite{khalifa_2021} and do important connections with RL theory. 
%     % \item Analysis of practical limitations
%     \item Propose modifications to the $GDC$ Algorithm proposed in \cite{khalifa_2021} to reduce variance in gradient estimation. (The use baseline). 
%     \item empirically, 
%     % \item Through a study we show intrinsic limitations of Finetuning Auto-regressive models in approximating constrained distributions and demonstrate the effectiveness of MC sampling in filling this gap.   
% \end{itemize}


==> RMvsDM NeurIPS 2022 Submission-5/sections/oldies (but goodies?)/similarities_differences_old.tex <==
If we define $\Ron \doteq \frac{P(x)}{\pit(x)}$, the expression \eqref{eq:dpgon} becomes very similar to \eqref{eq:REINFORCE}. 
In fact, should we equate $R(x)$ to $\Ron$, then the two expressions look almost identical.
Thus, the question that we address in this section is can we reduce DPG to PG by equating these two terms?
As we shall see, there are important nuances when drawing this analogy, which is only valid under certain conditions.

\paragraph{Distributional matching versus reward maximization}
Before digging into the question above, we first describe an alternative definition of the reward term.
Specifically, we could have been interested in finding a policy that maximizes the EBM ``score'' $P(x)$. Thus, in this case, we could simply define $R(x) = P(x)$ and follow \eqref{eq:REINFORCE}. 
Yet, this \emph{reward maximization} objective is maximized when the policy produces on a few (in the limit, one) sequence(s) having the highest score(s) $P(x)$. However, this objective would be totally unsuitable for (controlled) language modelling, where the goal is to approximate a \emph{distribution} over sequences, namely the normalized EBM distribution $p(x)$. It is also for this reason that $\Ron$ makes a better candidate to play the role of a ``reward'' term when matching distributions.

\paragraph{Gradients: superficially similar but inherently different}

Superficially, the expressions in the right-hand side of \eqref{eq:REINFORCE}: $\EX{x \sim \pit} R(x) \nabt \log \pit(x)$,  and of \eqref{eq:dpgon}: $\EX{x \sim \pit} \Ron \nabt \log \pit(x)$, look almost identical. However, the fact that $\Rt(x)$ depends on $\theta$ implies that, contrary to \eqref{eq:REINFORCE}, $\nabt \EX{x \sim \pit} \Ron \neq \EX{x \sim \pit} \Ron \nabt \log \pit(x)$.\footnote{
$\nabt \EX{x \sim \pit} \Ron = \EX{x \sim \pit} \left[ \Ron \nabt \log \pit(x) + \nabt \Ron \right]$.}

Actually, one can easily check that $\nabt \EX{x \sim \pit} \Ron = 0$. To confirm this, note that $\EX{x \sim \pit} \Ron$ is equal to the constant partition value $Z$, which does not depend on $\theta$:
\begin{align}
  \EX{\pit} \Ron &= \sum_x \pit(x) \frac{P(x)}{\pit(x)} \\
  &= \sum_x P(x) = Z. \label{eq:ZisConstant}
\end{align}
By contrast, in standard RL, $\EX{x \sim \pit} R(x)$ is of course strongly dependent on $\theta$: the whole point is to find $\theta$ that maximizes this expectation! A crucial consequence of that dependence is that DPG cannot be reduced down to RL by just defining $R(x) = \Ron$. The gradients of the cross-entropy objective in \eqref{eq:dpgon} will steer the policy in a different direction compared to the gradients of expected pseudoreward $\Ron$.\ftk{I added these two sentences to hopefully more clearly address the question whether DPG is RL \color{orange}{GK: yes, looks great to me!}}

\paragraph{Reducing variance of gradient estimates, the RL way}

While the objective of \eqref{eq:dpgon} is \emph{distribution matching}, and not \emph{reward maximization} as in RL, we also need to estimate $\EX{x \sim \pit} \Rt(x) \nabla_\theta \log \pit(x)$ at a \textbf{given} value of $\theta$, using a batch of samples $x$. For such a fixed $\theta$, we can define provisionally $R(x)\doteq \Ron$ and the problem of gradient estimation \emph{for this fixed $\theta$} is analogous to the estimation $\EX{x\sim \pit} R(x) \nabla_\theta \log \pit(x)$ based on a set of samples $x$ in standard RL.
Therefore, the techniques that have been developed to reduce the variance of the gradients estimates in RL can be ported to DPG insofar as we are computing the gradient estimates  \textbf{at a given $\theta$}.%
\footnote{To avoid confusion here, note that variance reduction methods for SGD focus on the objective of better estimating the true gradient expectation $\E_\pit [...]$, for a \emph{fixed} $\theta$. The fact that $\theta$ will then be \emph{updated} based on such estimates is orthogonal to this objective.}
% \gk{This point of setting $R(x)=\Ron$ is not clear to me, and seems contradictory to the previous discussion. MD: I added a footnote to try to clarify.}
%
In Section \ref{section:method}, we show how we can import one such variance reduction technique to DPG, namely the introduction of a ``baseline'', detailing its application to both \DPGon and \DPGoff algorithms.


\begin{comment}
% MD: Some material here could be used later. For now I am commenting it out.
  
Equations \eqref{eq:dpgon} and \eqref{eq:dpgoff} are equivalent to policy gradients methods in reinforcement learning (RL) \citep{sutton_policy_gradients} and our distinction between \DPGon and \DPGoff mirrors the distinction between on-policy and off-policy reinforcement learning \citep{Sutton2018}. To stress the connection, let us use the abbreviations $R^\text{ on}_\theta(x) = P(x)/\pit(x)$ and $R^\text{ off}_\theta(x) = P(x)/q(x)$ and call the corresponding terms in equations \eqref{eq:dpgon} and \eqref{eq:dpgoff} {\it pseudorewards}.

It is, however, equally important to stress out that our objective -- matching distributions by minimizing their divergence -- is {\it different} from the standard RL objective of maximizing expected reward. Moreover, unlike standard RL, $R^\text{ on}_\theta(x)$ does depend on policy parameters $\theta$ (the same applies to $R^\text{ off}_\theta(x)$ because the parameters of $q$ will usually be close to $\theta$). Finally, there is no notion of state in our formulation which prevents us from using value learning for variance reduction. In the next section we will show that despite those difference, we can extend formal framework proposed by \citeauthor{khalifa_2021} to exploit further insights from reinforcement learning and include a control variate reducing the variance of estimated gradients.
\end{comment}

==> RMvsDM NeurIPS 2022 Submission-5/sections/parametric_rewards.tex <==
\allowdisplaybreaks

Let us start with distinguishing between a ``parametric reward'' $\Rtheta$ which depends on $\theta$ and a standard reward $R$, which does not.
%
If we wished to maximize the expected parametric reward, $\E_{\pit} \Rtheta(x)$, 
we would follow its gradient, leading to the identities:
\begin{align}
    \nabt \E_{x \sim \pit} \Rtheta(x) &= \nabt \sum_x \pit(x) \Rtheta(x) 
    = \sum_x \pit(x) \nabt \Rtheta(x) + \sum_x \Rtheta(x) \nabt \pit(x) \\
    &= \sum_x \pit(x) \nabt \Rtheta(x) + \sum_x \pit(x) \Rtheta(x) \nabt \log \pit(x) \\
    &= \underbrace{\E_{x \sim \pit} \nabt \Rtheta(x)}_{\textrm{RG-term}} + \underbrace{\E_{x \sim \pit} \Rtheta(x) \nabt \log \pit(x)}_{\textrm{PG-term}}. \label{eq:two_terms}
\end{align}

Equation \eqref{eq:two_terms} is the sum of two terms: the first one, the ``RG-term" (Reward Gradient term), involves the gradient of the reward. The second one, the ``PG-term'' (Policy Gradient term), was obtained using the ``log derivative trick'' and involves the gradient of the policy \emph{stricto sensu}. In standard RL, where the reward does \emph{not} depend on $\theta$, the RG-term disappears and the gradient of expected reward consists solely of the PG-term. However, when $\Rtheta$ depends on $\theta$, the gradients are distinct (apart from specific cases where the RG-term evaluates to $0$, as we will see below).%, as is the case with \eqref{eq:dpgon}, the gradient directions are distinct. 



==> RMvsDM NeurIPS 2022 Submission-5/sections/repro_statement.tex <==
The source code for our experiments was based on the repository that \cite{khalifa_2021} published on GitHub.\footnote{\url{https://github.com/naver/gdc}} The two pretrained models used in our experiments are available on Hugginface Model Hub: \texttt{gpt}\footnote{\url{https://huggingface.co/gpt2}} and \texttt{mkhalifa/gpt2-biographies}.\footnote{\url{https://huggingface.co/mkhalifa/gpt2-biographies}} In addition to that, 

==> RMvsDM NeurIPS 2022 Submission-5/sections/rm_vs_dm.tex <==
In the previous section, we have summarized three approaches that have been suggested for fine-tuning language models. Two of them can be characterized as ``Reward Maximization'' (RM): Standard Policy Gradients (PG) and KL-control. On the other hand, DPG clearly belongs to the realm of ``Distribution Matching'' (DM) as it first defines the target distribution and then optimizes a policy to match it. In the rest of this section, we will explore connections between these two seemingly distinct concepts and, in the following section, we will exploit them to improve DM-based methods.

\subsection{Standard vs. Parametric Rewards}
\input{sections/parametric_rewards}
\subsection{KL-control as Distribution Matching}
\input{sections/klcontrol}

==> RMvsDM NeurIPS 2022 Submission-5/sections/similarities_differences_new.tex <==
In the previous subsection, we have connected KL-control, a method designed under a RM paradigm, to DM. Now, we turn to the converse question of whether DPG, a DM method, can be connected to RM.
We begin by noting that after defining $\Rt = \frac{P(x)}{\pit(x)}$, the DPG gradient $\EX{x \sim \pit} \frac{P(x)}{\pit(x)} \nabla_\theta \log \pit(x)$ acquires the format of the PG-term $\EX{\pit} \Rt \nabla_\theta \log \pit(x)$.

However, the DM objective of DPG \emph{cannot} be considered as maximizing the average ``reward'' $R_\theta(x) = \frac{P(x)}{\pit(x)}$, as this would require adding also the RG-term $\E_{\pit}\nabla_\theta \frac{P(x)}{\pit(x)}$ into the gradient, which in this case does not vanish. 

Nonetheless, the analogy 
%between 
\ptmd{behind}
this gradient term is more fruitful than it first appears.
As a matter of fact, DPG gradient estimates suffer from the same high-variance problems as with standard PG. While the objective of DPG (distribution matching) is different from that of Policy Gradients (reward maximization), DPG also needs to estimate the PG-term $\E_\pit \Rtheta(x) \nabt \log \pit(x)$ at a \emph{given} value of $\theta$, using a batch of samples $x$. 
% \fmd{Perhaps use the notation $\E_{\pi_{\theta_0}} R_{\theta_0}(x) \left. [\nabt \log \pit(x)]\right|_{\theta_0}$ to clarify the point.}
 For such a \emph{fixed} $\theta$, we can define provisionally set $R(x)\doteq \Rtheta$ and the problem of gradient estimation \emph{for this fixed $\theta$} is 
 % analogous
 \ptmd{identical}
 to the estimation $\EX{x\sim \pit} R(x) \nabla_\theta \log \pit(x)$ based on a set of samples $x$ in standard RL.
Therefore, techniques that have been developed to reduce the variance of the gradients estimates in RL can be ported to DPG insofar as we are computing the gradient estimates \emph{at a given $\theta$}. %
% last minute attempt to replace the following footnote by a later footnote
%\footnote{To avoid confusion, note that variance reduction methods for SGD focus on the objective of better estimating the true gradient expectation $\E_\pit [...]$, for a \emph{fixed} $\theta$. The fact that $\theta$ will then be \emph{updated} based on such estimates is orthogonal to this objective.} 
In Section \ref{section:method}, we show how one can import one such variance reduction technique to the DPG: baselines.
% detailing its application to both \DPGon and \DPGoff algorithms.

% \bigskip \bigskip \bigskip

% XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX

% \bigskip

% \paragraph{Distributional matching versus reward maximization}\fgk{Not sure what to do with this}

% Before digging into the question above, we first consider an alternative definition of the reward term.
% Specifically, we could have been interested in finding a policy that maximizes the EBM ``score'' $P(x)$. Thus, in this case, we could simply define $R(x) = P(x)$ and follow \eqref{eq:REINFORCE}. 
% Yet, this \emph{reward maximization} objective, in principle,\footnote{That is, barring the practical limitations imposed by the parametric family over $\theta$.} is optimized when the policy produces those few (typically, just one) sequence(s) having the highest score(s) $P(x)$. However, this objective would be totally unsuitable for (controlled) language modelling, where the goal is to approximate a \emph{distribution} over sequences, namely the normalized EBM distribution $p(x)$. 
% % Here, $\Rtheta$, which explicitly depends on $\theta$, makes a better candidate to play the role of a ``reward'' term when matching distributions.
% Interestingly, $\Rtheta$, by explicitly depending on $\theta$, makes it possible to achieve this goal, while still exploiting the PG-term $\E_\pit \Rtheta(x) \nabt \log \pit(x)$ along classical lines.



==> RMvsDM NeurIPS 2022 Submission-5/sections/variance_reduction.tex <==
\input{figures/tab_RLvsDPG}



%
%
Baselines are a standard variance reduction technique in the context of Policy Gradients \citep{Sutton2018}. The idea is to subtract from the reward $R(x)$ a value $B$ 
that does not introduce bias to the gradients but may change variance. After the introduction of baseline, equation \eqref{eq:REINFORCE} then takes the following form:
\begin{equation}
\label{pg_baseline}   
\nabt \EX{\pit} R(x) = \EX{\pit} [R(x)-B]\, \nabt \log \pit(x).
\end{equation}
%%


\begin{wrapfigure}{r}{0.4\textwidth}
    \vspace{-0.8cm}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/advantage-illustration.pdf} 
    \caption{
    \small{Values of reward, advantage and the baseline  for first 1000 epochs of a pointwise constraint experiment.}
    }
    \label{fig:advantage-illustration}
    % \vspace{-4cm}
\end{wrapfigure}

In standard RL, the simplest form of baseline $B$ is just the average of the rewards for the policy:\footnote{While this baseline is not optimal (proof Appendix \ref{appendix:optimal-baseline}), it is widely used in practice.}
\begin{equation}
    \label{eq:B_rl}
    B^{\text{RL}} = \E_{x \sim \pi_\theta} R(x).
\end{equation}


%
%
Following the same methodology of taking the baseline to be the expectation of the reward term, we can obtain a remarkably simple form of a baseline for DPG:
\footnote{In the scope of this paper, our focus is on  importing to DPG simple constant baselines. The advantage is that this is a technique that is not impacted by the fact that $R_\theta$ depends on $\theta$: it can be applied ``$\theta$-locally'' to provide a more accurate estimate of $\E_{x \sim \pit} R_\theta(x) \nabla_{\theta} \log \pit(x)$ for a \emph{fixed} $\theta$, irrespective of the values of $R_{\theta'}$ elsewhere, while variance reduction techniques that involve several $\theta's$ simultaneously raise additional challenges for parametric rewards.
}
\begin{equation}
 \label{eq:B}
\begin{aligned}
    B = \E_{x\sim \pit} \frac{P(x)}{\pit(x)} = \sum_x \pit(x) \frac{P(x)}{\pit(x)} = \sum_x P(x) = Z.
\end{aligned}
\end{equation}


\begin{fact}
\label{dpgon_baseline_unbiased}
Subtracting 
$B$ 
% $Z$
from $R_\theta(x)$ does not introduce bias into DPG gradient estimates.%
% last minute footnote attempt ...
% \footnote{One might be critical about our focus on just importing to DPG simple constant baselines of this sort when more sophisticated RL variance reduction techniques  such as TRPO, PPO, AC, ..., exist. However the advantage of the simple baseline is that it is a technique that is not impacted by the fact that $R_\theta$ depends on $\theta$: it is applied ``$\theta$-locally'' to provide a more accurate estimate of $\E_{x \sim \pit} R_\theta(x) \nabla_{\theta} \log \pit(x)$ for a \emph{fixed} $\theta$, irrespective of the values of $R_{\theta'}$ elsewhere. The other techniques are typically not $\theta$-local, and we leave them to further studies. 
%\footnote{One might be critical about 
%\footnote{In the scope of this paper, our focus is on just importing to DPG simple constant baselines of this sort while more sophisticated RL variance reduction techniques  such as TRPO, PPO, AC, ..., exist. However the advantage of the simple baseline is that it is a technique that is not impacted by the fact that $R_\theta$ depends on $\theta$: it is applied ``$\theta$-locally'' to provide a more accurate estimate of $\E_{x \sim \pit} R_\theta(x) \nabla_{\theta} \log \pit(x)$ for a \emph{fixed} $\theta$, irrespective of the values of $R_{\theta'}$ elsewhere. The other techniques are typically not $\theta$-local, and we leave them to further studies. 
%We leave more advanced importation techniques to further studies.


\end{fact}
\vspace{-10px}
\begin{proof}
Let us rewrite the DPG gradient in \eqref{eq:dpgon} with the added baseline $B=Z$:
\begin{equation}
\begin{aligned}
   \E_{x \sim \pit} \Big[ R_\theta(x) - Z \Big] \nabla_{\theta} \log \pit(x)
    &=\E_{x \sim \pit} R_\theta(x) \nabla_{\theta} \log \pit(x) 
    -Z \,\E_{x \sim \pit} \, \nabla_{\theta} \log \pit(x) \\
    &=\E_{x \sim \pit} R_\theta(x) \nabla_{\theta} \log \pit(x) 
    - Z \Big[\sum_{x} \nabla_{\theta} \pit(x) \Big]
\end{aligned}
\end{equation}
Here, the second term does not introduce bias because $Z \Big[\sum_x \nabt \pit(x) \Big]= 0$, leaving us with the exact same form of gradient as in the original DPG algorithm.
\end{proof}
%show 

%%%%%%%%%% algorithm 1 KLdpg + baseline %%%%%%%%%%%%%%
\input{figures/algorithm1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Z can be calculating globally
Note that since $B^{\text{RL}}$ depends on $\theta$, it has to be be re-estimated after each gradient update. On the other hand, $B$ does \emph{not} depend on $\theta$, which is an advantage because $B$ could be now estimated by averaging over samples from \emph{all} the different $\theta$'s without introducing bias, leading to a more accurate estimation. See Table \ref{tab:comparison_DPGvsPG} for a comparison of these two forms of baselines.\fmd{(4-10) About Table 1: in the caption you speak about $\nabt$ in the left column referring to the gradient of the loss function. I think this might be misleading (several forms of loss functions in our paper), what about replacing $\nabt$ in the first column with PG-term, or at least using PG-term terminology in the caption?}

%%%%%%%%%%%% DPG off %%%%%%%%%%%%%%%%%%%%%%%
The off-policy DPG version introduced in~\citep{opt-rl-arxiv-2019} and its KL-adaptive variant~\citep{khalifa_2021} sample a proposal distribution $q$ instead of the policy $\pit$. Then, the baseline takes the form
\begin{equation}
    \Boff = Z\frac{\pit(x)}{q(x)},
\end{equation}
where the $\frac{\pit(x)}{q(x)}$ term is an importance weight correcting for the bias introduced by sampling from~$q$. Similarly to the DPG case, we can prove the following (see Appendix~\ref{appendix:baselines}):
\begin{fact}
\label{dpgoff_baseline_unbiased}
Subtracting $\Boff$ from $R_\theta(x)$ does not bias the off-policy DPG gradient estimates.
\end{fact}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In practice, as shown on Figure~\ref{fig:advantage-illustration}, adding a baseline to KL-adaptive DPG  (\Algref{al:KL-adaptive-DPG-baseline}) centers the advantage %(defined as $A \doteq R_\theta(x)-B$)
\ptmd{(defined as $A \doteq  \frac{P(x)}{q(x)} - Z\frac{\pit(x)}{q(x)}$)}
around 0 leading to better performance on: convergence (section \ref{subsec:general_results}), stability on small batch sizes (section \ref{subsec:bsz_exps}), and variance reduction (section \ref{subsec:effectOnVarReduc}).


==> figures/table_bsz_experiments.tex <==
\begin{table}
\tiny
\begin{tabular}{lllrrrrrrrrr}
\toprule
             &      &      &  b(x) &  KL(p, pi) &  KL(pi, a) &  Dist-1 &  Dist-2 &  Dist-3 &  SB-3 &  SB-4 &  SB-5 \\
             & batch size & method &      &        &        &       &       &       &        &        &        \\
\midrule
word amazing & 0    & a & 0.00 &   6.46 &  -0.00 &  0.87 &  0.95 &  0.93 &   0.96 &   0.90 &   0.82 \\
             & 256  & GDC++ & 0.72 &   3.94 &   7.28 &  0.87 &  0.95 &  0.94 &   0.97 &   0.94 &   0.88 \\
             &      & GDC & 0.59 &   4.61 &   8.34 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             \
             & 512  & GDC++ & 0.72 &   2.57 &   5.34 &  0.86 &  0.95 &  0.93 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.69 &   2.40 &   5.36 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 1024 & GDC++ & 0.75 &   1.34 &   4.71 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.73 &   1.89 &   4.70 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 2048 & GDC++ & 0.73 &   1.35 &   4.33 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.71 &   1.46 &   4.40 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
\bottomrule
Multiple Dist & 0    & a & 0.12 &   0.16 &   0.00 &  0.90 &  0.95 &  0.92 &   0.98 &   0.94 &   0.90 \\
             & 256  & GDC++ & 0.24 &   0.65 &   1.06 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.52 &   1.04 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 512  & GDC++ & 0.24 &   0.37 &   0.78 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.36 &   0.88 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 1024 & GDC++ & 0.24 &   0.20 &   0.75 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.24 &   0.81 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 2048 & GDC++ & 0.24 &   0.20 &   0.68 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.22 &   0.70 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\

\bottomrule
\end{tabular}
\end{table}


==> sections/oldies (but goodies?)/intro.tex <==
%TODO: move somewhere else
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure1.pdf} 
    \caption{\small{
    Training trends of the Distributional Policy Gradient algorithm (DPG) for approximating Sequential Energy-Based Models. The addition of a \textit{baseline} reduces the variance of gradient estimates (left), leading to better convergence (right). 
    }}
    \label{fig:intro}
\end{wrapfigure}


With the advent of Large Language Models (LLMs), there has been a growing need for learning methods that require less data and for techniques to control the properties of the generated sequences, such as removing bias or harmful expressions~\citep{Bender_parrots,Bommasani:etal:2021}.
Sequential energy-based models (EBMs) have been recently recognized as a theoretically principled way of tackling these challenges by either injecting prior knowledge into these models \citep{A-parshakova-etal-2019-global,Deng2020Residual} or by imposing constraints upon them \citep{Naskar2020EnergyBasedRI,he-etal-2021-joint,khalifa_2021}. 
Describing their functioning in few words, they can represent constraints or prior knowledge about relevant features as sequence-level functions that can be combined with the model's own scores to describe an unnormalized distribution $P(x)$ over the space of possible sequences $x$.
However, whereas it is often simple to sample from an autoregressive language model, there is no obvious way to obtain samples from Sequential EBMs.

Distributional Policy Gradients (DPG)~\citep{opt-rl-arxiv-2019} are a family of learning algorithms that learn an autoregressive policy that approximates the probability distribution $p(x) = P(x)/Z$ induced by the EBM. 
In this way, it is possible to sample from the EBM by sampling from the autoregressive policy.
DPG was inspired by Policy Gradients (PG)~\citep{Williams92Reinforce}, a well-known technique in Reinforcement Learning. 
However, the extent to which the two approaches relate has not yet been thoroughly analyzed.
Establishing a formal connection between the two methods can have important consequences because if we succeed at it, DPG could benefit from a vast wealth of knowledge about PG that has been accumulated for over the past 30 years of research in RL.
In turn, this connection would directly impact all techniques built upon DPG.

In this paper, we make a detailed account of how the concept of reward, central to RL, translates into the DPG framework.
As a consequence, we can import well-established variance reduction techniques such as \emph{baselines}. 
We apply these insights to improve the GDC (Generation with Distributional Control) algorithm, a particular instantiation of DPG proposed by \citet{khalifa_2021} to \emph{control} language models.
This method is unique in allowing to define \emph{distributional} constraints on the language model while preventing \emph{catastrophic forgetting} of the original language model distribution.
Thanks to these properties, it can be applied to \emph{debiasing} the probability distributions of sequences containing mentions of different genders, among other usages such as constraining the topic or sentiment distribution.
Our results show a significant decrease in the variance of gradient estimates, thus obtaining improved constraint satisfaction, stability and sample efficiency.
Moreover, the improved algorithm has a much higher sample efficiency.
It can, for example, reach the performance that GDC achieves after $5$ million examples in half as many.


% Sequential energy-based models (EBMs) have been recently recognized as a theoretically principled way of injecting prior knowledge into autoregressive language models \citep{A-parshakova-etal-2019-global,Deng2020Residual} or of imposing constraints upon them \citep{Naskar2020EnergyBasedRI,he-etal-2021-joint,khalifa_2021}. 

% Sequential EBMs represent constraints or prior knowledge of relevant features as sequence-level functions that are combined with the scores of a language model to construct an unnormalized probability distribution $P(x)$.
% However, it is not clear how to obtain samples from the associated probability distribution $p(x) = P(x)/Z$ where $Z$ is the partition function.

%
% todo add more applications from ACL anthology papers
% EBM Cloze models~\cite{ClarkLLM20} 
%
% In this context, a sequential EBM $P(x) = a(x) b(x)$ is an unnormalized probability distribution over sequences $x$ which combines the probability scores of a base autoregressive model $a(x)$ with a nonnegative ``modifier'' $b(x)$ to express a preference towards certain sequences $x$. For instance, Generative Distributional Control or GDC~\citet{khalifa_2021} poses controllable language generation as a constraint satisfaction problem in which a pretrained language model is fine-tuned to approximate a target language model that fully satisfies some predefined constraints leading to an exponential expression for $b(x)$. Similarly, Global Autoregressive Models \citep{A-parshakova-etal-2019-global} and Residual EBMs \citep{Deng_EBM_20} enable data-efficient learning by augmenting an autoregressive language model with prior knowledge about its training data, expressed as preference towards certain sequences. In yet another line of work, \citet{Naskar2020EnergyBasedRI} augment a machine translation model $a$ with an energy-based reranker $b$: while $a$ was trained with maximum likelihood, $b$ prefers translations with high BLEU scores. In each case, $b(x)$ is flexible enough to represents requirements that couldn't be easily integrated in the training objective for $a$.

% The flexibility comes at a price: $P$ cannot be easily sampled from. This can be circumvented by training a second autoregressive model $\pit$ to approximate the normalized distribution $p$ associated with the target EBM $P(x)$. A family of algorithms, Distributional Policy Gradients (DPG), inspired by reinforcement learning (RL), was recently proposed as a solution to this approximation problem \citep{opt-rl-arxiv-2019,khalifa_2021}. Yet, the exact relation of DPG to Policy Gradients in standard RL remains poorly understood. In this work, we start by revisiting the motivations behind DPG and expose both fruitful connections but also important differences between DPG and standard RL. While RL typically tries to find a policy $\pit$ that maximizes the expected reward $\E_{x \sim \pit} R(x)$, DPG minimizes the distributional discrepancy (measured through cross-entropy) between an auto-regressive policy $\pit$ and the target EBM $P$. These two objectives imply similar functional forms of policy gradient estimates yet produce vastly different policies.

%  The connections we find between DPG and standard RL allow us to derive a DPG variant of \emph{baselines}, a popular variance reduction technique in standard RL \cite{suttonphd,williams1987}. In particular, we argue for a remarkably simple form of baseline: $Z = \sum_x P(x)$, the normalizing constant (partition function) associated with $P$. We empirically validate the benefits of adding such a baseline on an array of controllable language generation tasks such as constraining the topic, sentiment, or gender distribution of texts sampled from $\pit$. We observe a significant decrease in the variance of gradient estimates which translates into improved constraint satisfaction, stability and sample efficiency.
 
To summarize, the main contributions of the paper are:
% \vspace{-0.4cm}
\begin{itemize}
    \itemsep0em 
    \item A detailed comparison of the family of DPG algorithms with the policy gradients of standard RL,
    \item A theoretical justification for applying baselines --- a variance reduction technique from RL --- to DPG and a derivation of a particular choice of a baseline,
    \item An extensive empirical evaluation of the proposed algorithm --- DPG with baseline --- on controllable language generation tasks following the GDC approach, which results in more stable learning and higher sample efficiency.
\end{itemize}


%% some intro
% XXXX \\
% %%%
% a Sequential Energy based models - EBM over sequences. 
% %%%%
% In order to approximate a sequential EBM into an auto-regressive policy a recent class of algorithms referred to as Distributional Policy Gradients~\cite{A-parshakova-etal-2019-global} and its adaptive variants \cite{khalifa_2021} has been introduced.
% %
% This class of algorithms is intrinsically different in its objective to Standard Reinforcement Learning ones. It aims at minimizing the cross entropy objective between an auto-regressive policy $\pit$ and the underlying target distribution $p$ represented by the sequential EBM. While Standard Reinforcement Learning typically try finding a policy $\pit$ that maximize the expected reward $E_{\pit} R(x)$.
%


% Overall, our main contributions can be summarized as:
% \begin{itemize}
%     \item We revisit theory proposed in \cite{khalifa_2021} and do important connections with RL theory. 
%     % \item Analysis of practical limitations
%     \item Propose modifications to the $GDC$ Algorithm proposed in \cite{khalifa_2021} to reduce variance in gradient estimation. (The use baseline). 
%     \item empirically, 
%     % \item Through a study we show intrinsic limitations of Finetuning Auto-regressive models in approximating constrained distributions and demonstrate the effectiveness of MC sampling in filling this gap.   
% \end{itemize}


==> sections/oldies (but goodies?)/similarities_differences_old.tex <==
If we define $\Ron \doteq \frac{P(x)}{\pit(x)}$, the expression \eqref{eq:dpgon} becomes very similar to \eqref{eq:REINFORCE}. 
In fact, should we equate $R(x)$ to $\Ron$, then the two expressions look almost identical.
Thus, the question that we address in this section is can we reduce DPG to PG by equating these two terms?
As we shall see, there are important nuances when drawing this analogy, which is only valid under certain conditions.

\paragraph{Distributional matching versus reward maximization}
Before digging into the question above, we first describe an alternative definition of the reward term.
Specifically, we could have been interested in finding a policy that maximizes the EBM ``score'' $P(x)$. Thus, in this case, we could simply define $R(x) = P(x)$ and follow \eqref{eq:REINFORCE}. 
Yet, this \emph{reward maximization} objective is maximized when the policy produces on a few (in the limit, one) sequence(s) having the highest score(s) $P(x)$. However, this objective would be totally unsuitable for (controlled) language modelling, where the goal is to approximate a \emph{distribution} over sequences, namely the normalized EBM distribution $p(x)$. It is also for this reason that $\Ron$ makes a better candidate to play the role of a ``reward'' term when matching distributions.

\paragraph{Gradients: superficially similar but inherently different}

Superficially, the expressions in the right-hand side of \eqref{eq:REINFORCE}: $\EX{x \sim \pit} R(x) \nabt \log \pit(x)$,  and of \eqref{eq:dpgon}: $\EX{x \sim \pit} \Ron \nabt \log \pit(x)$, look almost identical. However, the fact that $\Rt(x)$ depends on $\theta$ implies that, contrary to \eqref{eq:REINFORCE}, $\nabt \EX{x \sim \pit} \Ron \neq \EX{x \sim \pit} \Ron \nabt \log \pit(x)$.\footnote{
$\nabt \EX{x \sim \pit} \Ron = \EX{x \sim \pit} \left[ \Ron \nabt \log \pit(x) + \nabt \Ron \right]$.}

Actually, one can easily check that $\nabt \EX{x \sim \pit} \Ron = 0$. To confirm this, note that $\EX{x \sim \pit} \Ron$ is equal to the constant partition value $Z$, which does not depend on $\theta$:
\begin{align}
  \EX{\pit} \Ron &= \sum_x \pit(x) \frac{P(x)}{\pit(x)} \\
  &= \sum_x P(x) = Z. \label{eq:ZisConstant}
\end{align}
By contrast, in standard RL, $\EX{x \sim \pit} R(x)$ is of course strongly dependent on $\theta$: the whole point is to find $\theta$ that maximizes this expectation! A crucial consequence of that dependence is that DPG cannot be reduced down to RL by just defining $R(x) = \Ron$. The gradients of the cross-entropy objective in \eqref{eq:dpgon} will steer the policy in a different direction compared to the gradients of expected pseudoreward $\Ron$.\ftk{I added these two sentences to hopefully more clearly address the question whether DPG is RL \color{orange}{GK: yes, looks great to me!}}

\paragraph{Reducing variance of gradient estimates, the RL way}

While the objective of \eqref{eq:dpgon} is \emph{distribution matching}, and not \emph{reward maximization} as in RL, we also need to estimate $\EX{x \sim \pit} \Rt(x) \nabla_\theta \log \pit(x)$ at a \textbf{given} value of $\theta$, using a batch of samples $x$. For such a fixed $\theta$, we can define provisionally $R(x)\doteq \Ron$ and the problem of gradient estimation \emph{for this fixed $\theta$} is analogous to the estimation $\EX{x\sim \pit} R(x) \nabla_\theta \log \pit(x)$ based on a set of samples $x$ in standard RL.
Therefore, the techniques that have been developed to reduce the variance of the gradients estimates in RL can be ported to DPG insofar as we are computing the gradient estimates  \textbf{at a given $\theta$}.%
\footnote{To avoid confusion here, note that variance reduction methods for SGD focus on the objective of better estimating the true gradient expectation $\E_\pit [...]$, for a \emph{fixed} $\theta$. The fact that $\theta$ will then be \emph{updated} based on such estimates is orthogonal to this objective.}
% \gk{This point of setting $R(x)=\Ron$ is not clear to me, and seems contradictory to the previous discussion. MD: I added a footnote to try to clarify.}
%
In Section \ref{section:method}, we show how we can import one such variance reduction technique to DPG, namely the introduction of a ``baseline'', detailing its application to both \DPGon and \DPGoff algorithms.


\begin{comment}
% MD: Some material here could be used later. For now I am commenting it out.
  
Equations \eqref{eq:dpgon} and \eqref{eq:dpgoff} are equivalent to policy gradients methods in reinforcement learning (RL) \citep{sutton_policy_gradients} and our distinction between \DPGon and \DPGoff mirrors the distinction between on-policy and off-policy reinforcement learning \citep{Sutton2018}. To stress the connection, let us use the abbreviations $R^\text{ on}_\theta(x) = P(x)/\pit(x)$ and $R^\text{ off}_\theta(x) = P(x)/q(x)$ and call the corresponding terms in equations \eqref{eq:dpgon} and \eqref{eq:dpgoff} {\it pseudorewards}.

It is, however, equally important to stress out that our objective -- matching distributions by minimizing their divergence -- is {\it different} from the standard RL objective of maximizing expected reward. Moreover, unlike standard RL, $R^\text{ on}_\theta(x)$ does depend on policy parameters $\theta$ (the same applies to $R^\text{ off}_\theta(x)$ because the parameters of $q$ will usually be close to $\theta$). Finally, there is no notion of state in our formulation which prevents us from using value learning for variance reduction. In the next section we will show that despite those difference, we can extend formal framework proposed by \citeauthor{khalifa_2021} to exploit further insights from reinforcement learning and include a control variate reducing the variance of estimated gradients.
\end{comment}

==> sections/repro_statement.tex <==
The source code for our experiments was based on the repository that \cite{khalifa_2021} published on GitHub.\footnote{\url{https://github.com/naver/gdc}} The two pretrained models used in our experiments are available on Hugginface Model Hub: \texttt{gpt}\footnote{\url{https://huggingface.co/gpt2}} and \texttt{mkhalifa/gpt2-biographies}.\footnote{\url{https://huggingface.co/mkhalifa/gpt2-biographies}} In addition to that, 
